SPEECHMINER: A Framework for Investigating and Measuring Speculative Execution Vulnerabilities

SPEculative Execution side Channel Hardware (SPEECH) Vulnerabilities have enabled the notorious Meltdown, Spectre, and L1 terminal fault (L1TF) attacks. While a number of studies have reported different variants of SPEECH vulnerabilities, they are still not well understood. This is primarily due to the lack of information about microprocessor implementation details that impact the timing and order of various micro-architectural events. Moreover, to date, there is no systematic approach to quantitatively measure SPEECH vulnerabilities on commodity processors. This paper introduces SPEECHMINER, a software framework for exploring and measuring SPEECH vulnerabilities in an automated manner. SPEECHMINER empirically establishes the link between a novel two-phase fault handling model and the exploitability and speculation windows of SPEECH vulnerabilities. It enables testing of a comprehensive list of exception-triggering instructions under the same software framework, which leverages covert-channel techniques and differential tests to gain visibility into the micro-architectural state changes. We evaluated SPEECHMINER on 9 different processor types, examined 21 potential vulnerability variants, confirmed various known attacks, and identified several new variants.

==> tex/02-background.tex <==
\section{Background}
\label{sec:background}

\subsection{Transient Execution Vulnerability}

Transient execution vulnerabilities are a category of micro-architectural bugs on modern pipelined processors that support speculative and out-of-order execution. To increase instruction-level parallelism, modern processors typically only enforce instructions retirement in program order to guarantee correctness of computation, but allow them to be executed in different orders. As a result of such performance optimization, instructions that should not be executed, \eg, due to branch target mis-prediction or exception raised in instructions before it in program order, would now have a short window of transient execution before they are discarded. Although transient execution will not cause permanent memory changes, side effects such as cache states would be altered but not reverted afterwards.

% \subsection{Software Fuzzers}

% Fuzzers are an automated security analyzing tools for software programs~\cite{}. Structured, but likely invalid and unexpected, inputs are generated automatically (sometimes with sources of randomness) and provided to the tested program. The program's execution is monitored to detect crashes or memory leaks, which may be used to indicate bugs in software.

% \yz{Yuan, categorization of fuzzing techniques should go here.}

==> tex/backup-05-understanding.tex <==
\section{Understanding \vulname Vulnerabilities}
\label{sec:understanding}

\yx{This section needs to be re-organized according to the logic of the whole paper. So first of all, the whole paper: 
[1] We would like to understand what leads to the success/failure of transient execution attacks. (This should be the takeaway but the current version does not answer well.) 
[2] To answer this question, We need to propose a two-phase fault handling model based on abstracted processor implementation to understand how the attacks exactly work. 
[3] We prove the correctness of our model by empirically showing that P1 determines fault handling and P2 determines squashing. 
[4] The two phases actually correspond to the two race conditions deciding the success of an attack: (i) data fetching vs. processor fault handling; (ii) instruction squashing vs. covert channel transmission. A good thing about our model is that we show these two race conditions can be considered separately. Then we have enough to answer the first question. The question turns into a more formal one: for each race condition, are we able measure/control the two racing parties? (Q1: measure = understand success/failure; Q2: control = create most favorable condition towards success)
[5] Consider race (ii) first. 
Q1 (baseline): we are able to measure the race condition by speculation window (we should well define it: number of instructions that still allow covert channel instruction to execute. notice its dependency on speculation primitive, since covert\_channel\_transmission=secret\_data\_delay+covert\_channel\_delay and we don't want to additionally prove secret\_data\_delay is constant).
Q2: we can control speculation window and we can prove it with the experiment: we can delay retirement using windowing gadget and speculation window grows accordingly ("accordingly" meaning linear growth). Thus, we can always ensure that race (ii) can be won and speculation window can be positive. (This is not 100\% logically strict because we cannot ensure the windowing gadget has absolutely no influence on the two parties of race (i). But I don't think people will be bothered by this point.)
[6] Consider race (i).
Q1 (baseline): we are able to measure both positive and negative relative latency. This is good because even if we answer no to Q2 (which is complex, see below), we can clearly understand it for sure.
Q2: This should be answered in three parts and all of are variant-specific, thus we provide the two case studies in <section 4.D-Tuning P1>.
Q2.1: Can we control data fetching without changing fault handling? Yes, data in L1/L2/LLC/memory/LFB/... And we can measure whether each is fast enough. For those variants whose P1 is not dependent on TLB (eg. segmentation fault), we can also control TLB.
Q2.2: Can we control fault handling without changing data fetching? That depends on the variant. Meltdown-US: No, data fetching also changes. Segmentation-limit: No, not changeable at all.
Q2.3: If some conditions (eg. TLB) change both factors at the same time, can we control them to influence the race condition? Meltdown-US: we can measure TLB changing with our tool and find that it does not help.
[7] We have systematically studied the race conditions for exploitation in one round of attack. The following question is whether the attacker is able to change those conditions that controls/influences the race condition.
How a sophiscated attacker can manipulate victim is beyond our scope, so we only study whether one round of attack itself benefits the race conditions of next round of attack.
Race (ii) can always be controlled by attacker so we only care about race (i). Recall our answers to Q2 of race (i), the only influencing condition we found was data fetching latency. We are unable to test buffers yet but we can test caching.
[8] Use our conclusions to explain known attacks and to clarify misunderstandings.
[9] As a bonus, we can apply the same framework on Spectre to do measurements and tests and discuss briefly about some conclusions.
[10] Discussion section fits here
[11] Related work, conclusion
}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{fig/tests.png}
% \caption{The overall organization of tests.}
% \label{fig:tests}
% \end{figure}

\vulname vulnerabilities are caused by speculative execution. However, being able to speculatively execute instructions itself does not qualify a vulnerability. 
The root cause of  \vulname vulnerabilities is that some inaccessible secret data could be accessed by speculatively executed instructions. Moreover, once the secret data is accessible to the speculative instructions, what can be done with it (\eg, leaking the secret using covert channels) is determined by the speculation window---the time period (in CPU cycles) of speculatively executing secret transmission instructions. 
Our two-phase fault handling model serves well in separating the two race conditions of (i) data fetching vs. processor fault handling and (ii) speculative instruction squashing vs. covert channel transmission. This allows a systematic understanding of what factors and how they determine the (in)exploitability of an attack.
Therefore, to understand \vulname vulnerabilities, their \textit{exploitability} and \textit{attack window} must be quantitatively measured. %\yx{TODO: make sure the term "attack window" is accurate}

\begin{packeditemize}

\item \textit{Understand effects of \phaseone and \phasetwo.}

\item Measure the \textit{exploitability} of \vulname vulnerabilities.

\item  Measure the attack windows of the \vulname vulnerabilities.

\item Study the side effects of speculative instructions (\eg, prefetching data). 

\end{packeditemize}

\yx{I took off the figure here. It does not make sense.}

The \sysname framework allows running each of the tests described in this section to examine different types of Speculation Primitives corresponding to different attack variants. For the clarification and simplicity of discussion, we illustrate these tests using a Speculation Primitive similar to the one used in the Meltdown-US attack~\cite{Lipp2018meltdown}. But it is worth noting the actual instruction sequences differ for distinct Speculation Primitives.





\subsection{Understanding Effects of \phasetwo}
\label{subsec:e2_effect}


This test is designed to determine the effects of \phasetwo on the entire execution engine. The experiments were conducted on an Intel i7-7700HQ machine with Ubuntu 16.04 (Linux 4.4.0-137) as the operating system. Each experiment is repeated for 5 times for reliability.

\begin{lstlisting}[float=htbp,caption={The effects of P2 on the execution engine.}, label={lst:squash}]
 // %RBX: address of uncached covert channel buffer
 // (%RBX-0x40): address of uncached data
 // *(%RBX-0x40) = %RBX
 // %RAX: address of some other uncached memory
 // %RCX: illegal address whose data is 0x42000
 // ---------------------------------------------
 // Windowing Gadget
     sub %rbx, %rax
     sub %rbx, %rcx
     sub $0x40, %rbx
     movq (%rbx), %rbx
 // ---------------------------------------------
 // Speculation Primitive
     movq (%rcx, %rbx, 1), %rcx
 // ---------------------------------------------
 // Disclosure Gadget
     [add $1, %rbx]
     [sub $1, %rbx]
     ...
     movq (%rbx), %rbx
\end{lstlisting}

\bheading{Instruction sequences.}
As shown in \lstref{lst:squash}, the instructions of the Disclosure Gadget are independent of the data read by the Speculation Primitive. However, because all instructions in the Speculation Primitive and the Disclosure Gadget are dependent on the data fetched in the Windowing Gadget, the Speculation Primitive and the Disclosure Gadget start at the same time. 


\bheading{Experiments and expected observations.}
In this test, the framework tunes the number of ADD/SUB instructions inserted in the Disclosure Gadget. If all issued instructions are eventually executed (\ie, not squashed at \phasetwo), we would expect to receive the covert-channel signal regardless of the number of inserted ADD/SUB instructions. Otherwise, the signal should disappear when the number of ADD/SUB instructions increases to a certain threshold.

\bheading{Results.}
In the experiment described in \secref{subsec:e2_effect}, we observed that when the inserted instructions exceed a threshold, the covert-channel receiver no longer receive any signal from the covert channel. As the number is much smaller than the size of ROB \cite{measuring-rob}, it is not cause by ROB limits. \hl{As a conclusion, \textit{issued instructions will be squashed due to an exception at \phasetwo. Any instruction not yet executed will not be executed at all.}}
In other words, \phasetwo determines the "attack window" for the secret to be transferred by covert channel. 

\begin{center}
\minibox[frame, rule=1pt,pad=3pt]{

\begin{minipage}[t]{0.95\columnwidth}
\textbf{Conclusion:} Issued instructions will be squashed due to an exception at \phasetwo. Any instruction not yet executed will not be executed at all.
\end{minipage}
}
\end{center}

%\framebox[\columnwidth]{As a conclusion, issued instructions will be squashed due to an exception at \phasetwo. Any instruction not yet executed will not be executed at all.}

\subsection{Understanding Effects of \phaseone}

Three sets of experiments were performed to understand the effects of \phaseone on the current execution unit, other execution units, and the entire execution engine, respectively. These experiments were conducted on an Intel i7-7700HQ machine with Ubuntu 16.04 (Linux 4.4.0-137) as the operating system. Each experiment is repeated for 5 times for reliability. %It is found that the conclusions made from the experiments are also true on all other tested processors. 

\subsubsection{\phaseone on Current Execution Unit}
\label{subsec:e1_existence}

This test is designed to determine how \phaseone affects the execution unit being used by the Speculation Primitive. 

\begin{lstlisting}[float=htbp,caption={The effects of \phaseone on the current execution unit.},label={lst:phaseonecurrent}]
 // %RBX: address of uncached covert channel buffer
 // (%RBX-0x40): address of uncached data
 // *(%RBX-0x40) = %RBX
 // %RCX: illegal address whose data is 0x42000
 // ---------------------------------------------
 // Windowing Gadget 
     sub %rbx, %rcx
     sub $0x40, %rbx
     movq (%rbx), %rbx
 // ---------------------------------------------
 // Speculation Primitive
     movq (%rbx, %rcx, 1), %rcx
 // ---------------------------------------------
 // Disclosure Gadget
     movq (%rbx, %rcx, 1), %rbx
\end{lstlisting}

\bheading{Instruction sequences.}
As shown in \lstref{lst:phaseonecurrent}, the instruction sequence consists of a Windowing gadget, a Speculation Primitive, and a Disclosure Primitive. The Speculation Primitive includes two SUB instructions to prepare the desired register values. Because all the subsequent instructions have dependency on the data read by the Windowing Gadget, they start to execute as soon as the data fetched by the Windowing Gadget becomes available, but not before that. 


\bheading{Experiments and expected observations.}
The tests were repeated four times, with the secret data placed in the L1 cache, L2 cache, the LLC, and the memory, respectively. The TLB entry of the secret address is always flushed to ensure a fixed \phaseone latency. In these experiments, we would hope to see whether the change of the data fetching latency affects the covert-channel signal received by the Disclosure Primitive. If so, whether \phaseone happens before the data is fetched affects the return values of current execution unit. 

\bheading{Results.}
We observed that only when the secret data is stored in the L1 cache could the correct covert-channel signal be received. When the secret data is store in L2, LLC, or the memory, a zero signal is received. This observation validates our theory in \ref{subsec:handling}. The execution unit stops execution after catching the exception; a dummy value of zero is returned as the result of the execution. %This process is what we define as \phaseone. 
\hl{Therefore, this experiment concludes that \textit{{\phaseone} terminates faulting instruction execution. If the latency of {\phaseone} is larger than the data fetching latency, the correct value can be propagated to the speculative instructions; otherwise, a zero value will be returned.}}


%\ignore{
%\subsection{Effect of \phasetwo on current execution unit}

%\bheading{Test goals.}
%In order to conclude that \phaseone is the sole factor that could stop the execution unit that triggers the exception, we need to prove that the data fetched has nothing to do with \phasetwo.

%\bheading{Experiments and expected observations.}
%\yx{here should be a simple experiment using code from \secref{subsec:e2_change} but observe whether the captured value change from the correct value to zero. The result is included in \secref{subsec:e2_change_eval}.}
%}


\subsubsection{\phaseone on Other Execution Units}
\label{subsec:e1_effect}
This test aims to determine whether \phaseone affects other execution units. If that is the case, attacks may be enhanced by combining two or more Speculation Primitives.

\bheading{Instruction sequences.}
Different from other tests, two Speculation Primitives are included in this test to determine whether \phaseone of the first Speculation Primitive also influences the execution unit used by the second Speculation Primitive. We consider two cases, depending on whether the two Speculation Primitives access the same memory address.

First, the two Speculation Primitives access the same memory address. The instruction sequence is designed as shown in \lstref{lst:sameaddress}. A sequence of inter-dependent ADD/SUB instructions are inserted between the two Speculation Primitives to control the delay of the execution of the second Speculation Primitive. Since the first inserted ADD instruction and the first Speculation Primitive both have data dependency on the Windowing Gadget, they start at the same time. But the second Speculation Primitive has to wait until all the inserted ADD/SUB instructions finish. The Disclosure Gadget is used to measure the speculation window of the second Speculation Primitive. 

\begin{figure}[tb]
\centering
\includegraphics[width=\columnwidth]{fig/phaseone_on_other.png}
\caption{Illustration of \phaseone effects on other execution units.}
\label{fig:phaseone_on_other}
\end{figure}

Second, the two Speculation Primitives access different memory addresses. The instruction sequence used is the same as the first case, except that the memory addresses accessed by the two Speculation Primitives are different. 



\begin{lstlisting}[float=htbp,caption={The effects of P1 on the other execution units},label={lst:sameaddress}]
 // %RBX: address of uncached covert channel buffer
 // (%RBX-0x40): address of uncached data
 // *(%RBX-0x40) = %RBX
 // (%RBX+0x3000): address of uncached data
 // %RCX: illegal address #1 whose data
 // %RAX: illegal address #2 whose data is 0x42000
 // ---------------------------------------------
 // Windowing Gadget
     sub %rbx, %rax
     sub %rbx, %rcx
     sub $0x40, %rbx
     movq (%rbx), %rbx
 // ---------------------------------------------
 // Speculation Primitive #1
     movq (%rcx, %rbx, 1), %rcx
 // ---------------------------------------------
 // special inserted instructions for the experiment
     add %rbx, %rax
     [add $1, %rax]
     [sub $1, %rax]
     ...
 // ---------------------------------------------
 // Speculation Primitive #2
     movq (%rax), %rax
 // ---------------------------------------------
 // Disclosure Gadget
     movq (%rbx, %rax, 1), %rbx
\end{lstlisting}

\bheading{Experiments and expected observations.} In both tests, the relevant data are stored in the L1 cache. As shown in \figref{fig:phaseone_on_other}, the events with black labels describe the first Speculation Primitive, and the ones with blue labels describe the second. By delaying the execution of the second Speculation Primitive, \phaseone of the first Speculation Primitive can happen before the second Speculation Primitive fetches the secret data. Therefore, in the experiment, we gradually inserted more instructions between the two Speculation Primitive to delay the start of the second Speculation Primitive. 

\bheading{Results.}
In both experiments, regardless of whether the two Speculation Primitives accesses the same memory addresses or not, by gradually inserting instructions between them, we never witnessed that the received covert-channel signal changes from the correct value to zero. Instead, we only observed that after some threshold, the signal disappears. This is because \phaseone of the first Speculation Primitive does not influence the other execution units (by zeroing their results) but its \phasetwo does (by squashing their execution).
\hl{To conclude, \textit{{\phaseone} of the first Speculation Primitive does not affect other execution units.}} This also means there is no need to specially consider attacks that place two Speculation Primitives next to each other to improve the attacks.



\subsubsection{\phaseone on Execution Engine}
\label{subsec:e1_exec}

In this test, we hope to confirm that \phaseone does not influence other components of the execution engine, \ie, squashing speculative instructions in ROB and/or the altering code fetching in the front end, which determines the speculation window.

\bheading{Instruction sequences.}
The instruction sequence design is close to \lstref{lst:squash}. The only difference is that after Line 11, one memory load instruction (\ie, movq (\%rax, \%rbx, 1), \%rax) is added. 

\bheading{Experiments and expected observations.}
The strategy of the test is to change the latency of \phaseone while fixing the latency of \phasetwo. If the measured speculation window does not change according to \phaseone latency, \phaseone has no effect on the entire execution engine.

To change the latency of \phaseone, we control the TLB status of the page storing the secret data---by preloading or flushing the TLB entry. In this way, \phaseone of the Speculation Primitive changes accordingly. 

To fix \phasetwo latency, one additional memory load instruction is added in the windowing gadget, which begins to execute at the same time as the Speculation Primitive and the Disclosure Gadget. The goal of this instruction is to delay the retirement of all subsequent instructions, so that the retirement of the Speculation Primitive waits on the retirement of this memory load instruction. In this way, the \phasetwo latency is not determined by the the Speculation Primitive itself, which is changed because the TLB entry of the secret data page is preloaded or flushed, but by the retirement of the memory load instruction. To achieve this goal, the data to be loaded by this instruction is placed in the L2 cache and the TLB of the corresponding page is flushed.  


\bheading{Results.}
When changing the \phaseone latency, we did not observe any changes in the speculation window. %\hl{Therefore, we conclude that \textit{{\phaseone} has no influence on the entire execution engine}}.

\begin{center}
\minibox[frame, rule=1pt,pad=3pt]{

\begin{minipage}[t]{0.95\columnwidth}
\textbf{Conclusion:} \phaseone terminates the current execution unit but has not effects on other execution units or the entire execution engine.  
\end{minipage}
}
\end{center}


\subsection{Measuring \vulname Exploitability}
\label{subsec:e1_measure}

This test aims to determine whether a given variant of \vulname is exploitable, by measuring the relative latency of \phaseone and data fetch. If \phaseone comes sooner, the processor is not vulnerable with regard to the underlying Speculation Primitive. 

We performed tests on 9 machines (2 laptops, 5 desktops and 1 cloud VM). All tested machines run Ubuntu 16.04 with Linux kernel 4.4.0-137 (or 4.4.0-141 for compatibility issues on newer hardware) and KPTI is turned off. %KPTI as a software patch may make our study on the PTE-US variant inaccurate.
All the Intel microcode versions are rolled back to version 20171117 (except for Coffee Lake, which does not have older microcode, and the cloud VM, which we cannot control). %to make sure later microcode patch does not influence our tests. The only two exceptions are with Coffee Lake (no old microcode) and cloud VM (no control over microcode). But the tests on these two machines also show no influence by the microcode patch. 
The AMD microcode version is 3.20180515.1. The test can be extended to patched microcode and countermeasures, such as KPTI \yz{XXXX}. We would like to open source \sysname to enable other researchers to perform tests in other settings.

%We do not test all machines with up-to-date microcode patch because the core of our study is to understand the true nature of \atknames systematically on hardware level. The tool may also be useful in verifying the effectiveness of patches, but this is not within the scope of this paper.

\bheading{Instruction sequences.}
As shown in \lstref{lst:exploitability}, the Windowing Gadget has a memory load instruction that retires slowly due to long latency of memory access, but it does not have dependency on the previous instructions, nor does any subsequent instructions depend on it. It is used to ensure that the retirement of the Speculation Primitive (the \phasetwo latency) is sufficiently delayed. 

\begin{lstlisting}[float=htbp,caption={Exploitability test with \phaseone measurement.},label={lst:exploitability}]
 // %RBX: address of uncached covert channel buffer
 // (%RBX-0x40): address of uncached data
 // *(%RBX-0x40) = %RBX
 // %RCX: illegal address whose data is 0x42000
 // ---------------------------------------------
 // windowing gadget
     movq %rbx, %rax
     sub $0x40, %rax
     movq (%rax), %rax
 // ---------------------------------------------
 // speculation primitive
     movq (%rcx), %rcx // could be any illegal inst.
 // ---------------------------------------------
 // disclosure gadget
     movq (%rbx, %rcx, 1), %rbx
\end{lstlisting}

\bheading{Experiments and expected observations.}
Each tested instruction sequence was executed under a variety of conditions, with varying data access latency (cached in L1, L2, or LLC) and address translation latency (whether or not TLB entries are created for the corresponding pages). \sysname is able to enumerate all possible combinations to achieve the optimal condition. In each test, if the Disclosure Primitive receives the correct signal from the covert channel, the vulnerability is exploitable. Otherwise, if a zero signal is received, the vulnerability is not exploitable as the \phaseone latency is shorter than data available latency. However, if no signal can be received, speculation is not allowed. 



%\subsubsection{Exploitability}

\begin{table*}[tb]
\begin{center}
{\scriptsize
\begin{tabular}{p{0.34\columnwidth}|p{0.13\columnwidth}|p{0.13\columnwidth}| p{0.14\columnwidth}|p{0.14\columnwidth}|p{0.16\columnwidth}|p{0.13\columnwidth}|p{0.12\columnwidth}|p{0.15\columnwidth}|p{0.13\columnwidth}}
 & Laptop 1 & Laptop 2 & Desktop 1 & 
Desktop 2 & Desktop 3 & Desktop 4 & Desktop 5 & Desktop 6 & Cloud 1 \\ 
Variant & KabyLake & KabyLake & Haswell-EP & SandyBridge & Westmere-EP & CoffeeLake & KabyLake & AMD EPYC & Skylake-SP \\
\toprule

PTE (Present) & Y & N/A & N/A & N/A & N/A & Y & Y & N/A & Y \\ \hline

PTE (Reserved) & Y & N/A & N/A & N/A & N/A & Y & Y & N/A & Y \\ \hline

PTE (US) & Y & Y & Y & Y & Y & Y & Y & R & Y \\ \hline

Load CR4 & R & R & R & R & R & R & R & R & R \\ \hline

Load MSR (0x1a2) & R & R & R & R & R & R & R & N/A & N/A \\ \hline

Protection Key (User) & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & Y \\ \hline

Protection Key (Kernel) & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & Y \\ \hline

SMAP violation & Y & Y & N/A & N/A & N/A & Y & Y & Y* & Y** \\ \hline

PTE (write w/ RW=0) & Y & Y* & Y & Y & Y & Y & Y & R & Y \\ \hline

Load xmm0 (CR0.TS) & Y & Y & Y & Y & Y & Y & Y & N/A & N/A \\ \hline

BOUND (32-bit) & Y & Y & Y & Y & Y & Y & Y & Y & Y \\ \hline

DS Over-Limit (32-bit) & N & N & N & N & N & N & N & Y & N \\ \hline

SS Over-Limit (32-bit) & N & N & N & N & N & N & N & Y & N/A \\ \hline

DS Not-Present (32-bit) & R & R & R & R & R & R & R & R & R \\ \hline

SS Not-Present (32-bit) & R & R & R & R & R & R & R & R & R \\ \hline

DS Execute-Only (32-bit) & R & R & R & R & R & R & R & R & R \\ \hline

CS Execute-Only (32-bit) & R & R & R & R & R & R & R & R & R \\ \hline

DS Read-Only (write, 32-bit) & Y & Y & Y & Y & Y & Y & Y & R & Y \\ \hline

SS Read-Only (32-bit) & R & R & R & R & R & R & R & R & R \\ \hline

DS Null (32-bit) & N & N & N & N & N & N & N & R & N \\ \hline

SS Null (32-bit) & R & R & R & R & R & R & R & R & R \\ \hline

SS $DPL \neq CPL$ (32-bit) & R & R & R & R & R & R & R & R & R

\end{tabular}
}
\end{center}
\vspace{-10pt}
\caption{Exploitability evaluation on different machines. Y: exploitable. N: non-exploitable. R: no speculative execution. N/A: unable to test. Y*: both expected data and zero data are captured in all covert channel reloads. Y**: the only exploited case with success rate not 100\% (about 60\%). Laptop 1: i7-7820HQ (Kaby Lake). Laptop 2: i7-7700HQ (Kaby Lake). Desktop 1: Xeon E5-1607v3 (Haswell-EP). Desktop 2: i3-2120 (Sandy Bridge). Desktop 3: Xeon E5620 (Westmere-EP). Desktop 4: Xeon E-2124G (Coffee Lake). Desktop 5: i7-7700 (Kaby Lake). Cloud 1: Amazon EC2 C5 instance. Desktop 6: AMD EPYC 7251.}
\label{tbl:exploitability}
\end{table*}

\bheading{Results.}
The results are shown in \tabref{tbl:exploitability} and a reference of the tested variant names to their description can be found in \appref{sec:exception_list}. Some variants are unable to be tested due to lack of hardware support or OS support on certain machines and they are marked as N/A. On the tested Intel machines, Meltdown-US (accessing supervisor memory page from user space) and Meltdown-RW (writing to a read-only memory page) are exploitable while the AMD machine shows no speculation. When testing Meltdown-Present (\texttt{Present} flag cleared) and Meltdown-Reserved (\texttt{Reserved} flag set), signal handler cannot be used since the whole OS will crash. Thus, only the machines also equipped with Intel TSX~\cite{inteltsx} are tested and reported. Loading restricted registers (CR4 and MSR) on all tested machines show that no speculative load is allowed. Meltdown-MPK (bypassing the restriction of memory protection keys) could only be tested on Amazon EC2 E5 instance and it was found exploitable. Meltdown-FP (accessing a lazy-context-switch float pointer register) is also found exploitable on Intel machines. Meltdown-BR ( accessing an array with an over-range index) is found exploitable on all tested machines although the BOUND instruction raises an exception when it discovers the violation. In 32-bit mode, segmentation is enabled and thus relevant variants could be tested. Most of them are not exploitable or does not allow further speculation at all, since paging checks has to wait until segmentation translation produces a linear address while segmentation check begins at the same time as the translation. However, still some of them are found exploitable on either Intel or AMD platform.

%One new variant on this basis is discovered and will be explained shortly. Meltdown-SMAP, also a newly found variant, is possible to be expoited on all testable platforms and we will explain it in more details. 



%We find that among the 100,000 rounds of repeated tests in all tested variants, at most one of the covert channel buffer entries could be touched. And when one of them (either corresponding to the correct data or to zero) shows a hit, the hit rate is above 99\%.

In our experiments, a few new variants were found by the \sysname framework. \textit{We have reported these new variants to Intel and AMD already.}

\begin{itemize}
\item \textit{Supervisor mode access violating SMAP (Intel \& AMD).}
Supervisor Mode Access Prevention (SMAP) forbids code in the kernel mode from accessing to user-space addresses.  However, as shown in \tabref{tbl:exploitability}, on some of our tested machines, SMAP can be bypassed using speculative execution when the secret data is in the L1 cache. When the data is in lower-level caches, zero signal is captured. %In fact, for all the new and known exploitable cases with the one-load-instruction model, we found that they were exploitable only when the secret data was in L1 cache. Presence of TLB entry does not influence exploitability in the case of SMAP. 

\item \textit{Supervisor mode access bypassing MPK (Intel).}
When a user space page is set to be inaccessible using Memory Protection Key (MPK), its accesses from kernel code is also forbidden, which triggers a page fault exception. However, as demonstrated on the tested cloud server (see \tabref{tbl:exploitability}), if the secret data is already in the L1 cache, it can be leaked through speculatively executed Disclosure Gadget. 

\item \textit{Memory writes to read-only data segments (Intel).}
Segmentation is used in the 32-bit mode. However, memory writes to a read-only data segments can be speculatively used by following instructions. In this case, the caching and TLB status does not affect the exploitability. This vulnerability is similar to the \texttt{Meltdown-RW} \cite{}, but its security implication is different: \texttt{Meltdown-RW} takes advantage of store-to-load forwarding. As the store buffer is indexed by the linear address (not logical address), the forwarding is speculative as the logical-to-physical translation is not yet finished. Therefore, it is not surprising that the permission check (using flags in the PTE) happens after the store-to-load forwarding. However, in contrast, the segmentation check is performed during the translation from logical addresses to linear addresses. Thus, when the store buffer queues the store instruction to the given linear address \cite{US6378062}, the segmentation access privilege check should already be done. However, our test suggests that this is not the case as a following load could directly use the store value. This validates the conclusion of the recent Fallout attack \cite{} that store buffers predict aggressively using only the lowest bits of addresses.



\item \textit{Reading from a logical address over the limit of segment (AMD).}
When tested in 32-bit mode, a load to a logical address beyond the segment limit is forbidden, which triggers an exception. However, we have found that the segmentation check can be bypassed by speculative execution. The vulnerability is exploitable when the TLB entry of the page is present and the data is cached in the L1 cache. The same vulnerability cannot be found in Intel processors.

\end{itemize}







\subsection{Measuring and Tuning \phaseone and \phasetwo}

%The next question we explored is whether \phaseone and \phasetwo can be tuned.\yz{TODO: say something nice here}




\subsubsection{Measuring and Tuning \phaseone Latency}
\label{subsec:e1_change}

This test aims to quantitatively measure the relative latency of \phaseone, compared to data fetching. 



\begin{lstlisting}[float=htbp,caption={Quantitative measurement of \phaseone latency},captionpos=b,label={lst:framework2}]
 // %RBX: address of uncached covert channel buffer
 // %RCX: illegal address whose data is 0x42000
 // ---------------------------------------------
 // Suppressing Primitive
     [movq (%rax), %rax] // legal access
     [movq (%rax), %rax] // legal access
     ...
     movq (%rax), %rax // suppressing w/ exception
 // ---------------------------------------------
 // Speculation Primitive
     movq (%rcx), %rcx // could be any illegal inst.
 // ---------------------------------------------
 // Disclosure Gadget
     [add $1, %rcx]
     [sub $1, %rcx]
     ...
     movq (%rbx, %rcx, 1), %rcx
\end{lstlisting}

\bheading{Instruction sequences.}
The construction of the instruction sequence is different from other tests as a \textit{Suppressing Primitive} is needed in the test. The Suppressing Primitive precedes all other components in order to conceal the effect of executing the \pluginonename. This is achieved by ensuring that the instructions executed in all other components never retire. In the example of \lstref{lst:framework2}, the Suppressing Primitive is simply an illegal memory load from address 0, but it can also be implemented using conditional branches, indirect jumps, or retpoline. The Suppressing Primitive creates a fixed speculation window for the rest of the instruction sequence to execute. Because it is desired that this speculation window is greater than the one created by the Speculation Primitive, the Suppressing Primitive includes a few memory loads before the faulting instruction and leverages the pointer chasing technique~\cite{pointerchasing} to further enlarge its speculation window. The speculation window cannot be longer than the size of the ROB.

\begin{wrapfigure}{r}{0.6\columnwidth}
\includegraphics[width=\linewidth]{fig/atk_window_xmm_.eps}
    \caption{Size of the effective Windowing Gadget vs. speculation windows.}
    \label{fig:atk_window_xmm}
\end{wrapfigure}

A type-II Disclosure Gadget is used; all its instructions depend on the Speculation Primitive. Thus, the Disclosure Gadget only begins execution after the data is returned from the Speculation Primitive, regardless of its correctness. 


\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{fig/e1_latency.png}
\caption{Illustration of quantitatively measurement of \phaseone latency.}
\label{fig:e1_latency}
\vspace{5pt}
\end{figure}

\bheading{Experiments and expected observations.}
By flushing the secret data to memory, the framework ensures that a zero data is returned by the Speculation Primitive. Let $T_{P1}$ be the number of cycles to retrieve the zero data by the Speculation Primitive, $T_{spec1}$ be the speculation window of the Suppressing Primitive, and $T_{delay}$ be the latency for the Speculation Primitive to begin execution, which are both fixed. The number of inserted instructions in the Disclosure Gadget is tuned to determine $T_{spec2}$, which is the speculation window of the Speculation Primitive. As the Disclosure Gadget starts after the Speculation Primitive has retrieved the data, we have $T_{delay} + T_{P1} + T_{spec2} = T_{spec1}$ (shown in \figref{fig:e1_latency}).

To estimate $T_{P1}$, a control test is run. In the control test, the Speculation Primitive accesses a legal data, which does not trigger exceptions. But still, the execution will be reverted due to the Suppressing Primitive. In this case, the number of cycles to retrieve the legal data is $T_{data}$. With all other conditions unchanged, we have $T_{delay} + T_{data} + T_{spec2'} = T_{spec1}$. Without the need of calculating the exact values of $T_{spec1}$ and $T_{delay}$, the relationship between $T_{data}$ and $T_{P1}$ can be estimated in a differential manner: $T_{data} - T_{P1} = T_{spec2} - T_{spec2'}$.

\bheading{Results.}
We ran the tests on Meltdown-US as an example and found that $T_{data} - T_{P1} = 0$, which means \phaseone and L1 cache data fetching arrives at the same cycle. This also explains why most attacks cannot work when the data is in higher-level caches (unless the effects of prefetching is exploited, see \secref{subsec:prefetch}).  %\yx{added a sentence here} The data further answer the common question of why Meltdown-US attacks often capture zeros as the results. In real-world attack settings with no intentional interference, the likelihood for the secret data to be in L1D is much lower than in L2, LLC or memory.


%The test described in \lstref{lst:framework2} enables quantitative analysis of the vulnerability. It helps us explain why some vulnerabilities are exploitable and others are not. For instance, when the Speculation Primitive is a kernel memory read from userspace, the L1 data fetching latency is smaller than the latency of \phaseone, so the correct value can be leaked. 



We also performed the tests on negative results in \tabref{tbl:exploitability}. For example, when accessing data beyond the segment limit, data in \tabref{tbl:exploitability} suggest the vulnerability is not exploitable. By running the test to quantitatively measure $T_{P1}$, we were surprised by find out that $T_{data} - T_{P1} = 0$, which means \phaseone come right before the data is available.  
However, when data is available in the L2 cache, we find $T_{data} - T_{P1} = -12$, which suggests \phaseone come 12 cycles earlier than the data is available. Due to \sysname's ability to quantitatively measure a negative relative \phaseone latency, we are able to deterministically claim the inexploitability of certain variants on given hardware. This completely changes the view towards the security against \vulname.

\bheading{Tuning \phaseone.}
The test described in \lstref{lst:framework2} also enable us to reason about whether \phaseone of a Speculation Primitive can be delayed by changing the instruction sequences. This is critical as it matters to whether the exploitability of a vulnerability can be manipulated by software.

In the Speculation Primitives that involves exceptions raised by permission checks in PTEs, the absolute \phaseone latency (execution of the instruction to \phaseone) includes two components: TLB entry loading and permission checking. Similarly, the absolute latency of data fetching (execution of the instruction to data ready) also includes two components: TLB entry loading and data fetching. Therefore, the relative \phaseone latency (data available to \phaseone) only depends on the latency of permission checking and that of data fetching, both of which happens after the TLB entry is ready. Therefore, by altering TLB status, the relative \phaseone latency cannot be changed. We have verified this discussion in the test described in \lstref{lst:framework2}. When keeping the cache status of the secret data unchanged, it is found that the relative \phaseone latency remains the same in the experiments.


In the Speculation Primitives that involves exceptions raised by other checks, however, the relative \phaseone latency can be changed. For example, when the exception is raised by segmentation fault, the absolute \phaseone latency has nothing to do with TLB loading, because the exception is raised before page-level checking; however, the data fetching latency can be delayed by flushing TLBs. Therefore, the relative latency of \phaseone can be decreased by TLB preloading. Therefore, the optimal attack is represented by the condition with TLB entries present and secret data in the L1 cache. If in the optimal attack, the data fetching fails to outrun \phaseone, the vulnerability is not exploitable. In the experiment, flushing the TLB entries (compared to preloading them) leads to a decrease of the relative \phaseone latency of over 100 cycles.



%\subsubsection{Quantitative Measurement of \phaseone Latency}
%\label{subsec:e1_change_eval}
For the tests that yield $Y$ or $N$ in \tabref{tbl:exploitability}, further analysis can be conducted in test described in \secref{subsec:e1_change}. The only exceptions are when a \texttt{reserved} flag is set or the \texttt{present} flag is cleared. They can fetch neither correct data nor zero when using a suppressing primitive. The terminal faults seem to also be terminating the handling of the suppressing primitive. They can only be exploited when wrapped with a TSX transaction. \yx{is this clearer?}


\subsubsection{Measuring and Tuning \phasetwo Latency}
\label{subsec:e2_change}

This test aims to determine whether the latency of \phasetwo can be changed, and if so, how. 

\begin{lstlisting}[float=htbp,caption={Tuning \phasetwo latency.},label={lst:retirement}]
 // %RDI: address of uncached covert channel buffer
 // %RSI: illegal address whose data is 0x42000
 // ---------------------------------------------
 // Windowing Gadget
     movapd \%xmm0, \%xmm1
     addpd \%xmm1, \%xmm0
     [cpuid]
     mulpd \%xmm1, \%xmm0
     ...
     movapd \%xmm0, \%xmm1
     addpd \%xmm1, \%xmm0
     mulpd \%xmm1, \%xmm0
 // ---------------------------------------------
 // Speculation Primitive
     movq (%rsi), %rax
 // ---------------------------------------------
 // Disclosure Gadget
     [add $1, %rax]
     [sub $1, %rax]
     ...
     movq (%rdi, %rax, 1), %rax
\end{lstlisting}



\bheading{Instruction sequences.}
The instruction sequence is shown in \lstref{lst:retirement}.
As the retirement of the Speculation Primitive only happens after that of the Window Gadget, the strategy is to delay the latter. The Windowing Gadget consists of 25 repeated sequences of three SSE2 instructions: MOVAPD, ADDPD and MULPD---thus 75 instructions in total. These floating point instructions are slow but can be executed in parallel with the Speculation Primitive and the Disclosure Gadget. Each of these floating point instructions has data dependency on its predecessor. 

To fine tune the retirement of the Speculation Primitive, a CPUID instruction is inserted in the Windowing Gadget. As the CPUID instruction serializes the execution of the instructions before and after it (\ie, no instruction is issued before CPUID retires), only the floating point instructions after CPUID are effective in the Windowing Gadget. Therefore, the retirement of the Speculation Primitive is further delayed if there is CPUID is inserted earlier in the floating point instructions; and vice versa.

%Given the fixed sequence, we control the EFFECTIVE windowing gadget by inserting a CPUID instruction inside the sequence since CPUID serializes execution. For example, if we want no windowing gadget at all with a clean ROB, we insert CPUID at the end of the windowing gadget sequence, right before the speculation primitive. Or if we want a length of 75, we put CPUID at the beginning of the windowing gadget sequence.

The Disclosure Gadget is of type-II. All instructions are dependent on the Speculation Primitive.

%The reason is that we force the TLB availability and cache status to be constant, making the execution time of the speculation primitive to be always the same. We only care about the changing trend of the speculation window but do not need to measure its exact length.

\bheading{Experiments and expected observations.}
For each position in the Windowing Gadget where CPUID is inserted, the framework automatically alter the number of ADD/SUB instructions to identify the speculation window. In this way, the correlation between \phasetwo and the attack window can be observed. It also answers the question whether the attack window can be changed.

\bheading{Results.}
In \figref{fig:atk_window_xmm}, the x-axis is the effective size of Windowing Gadget (tuned by moving the position of CPUID) and the y-axis is speculation window. By gradually moving the position of CPUID from the beginning of the Windowing Gadget to the end, which changes the effective length of Windowing Gadget, the speculation window also grows accordingly. Therefore, we conclude that \textit{\phasetwo latency can be increased}. Prior studies~\cite{Lipp2018meltdown} have reported the attack window of certain attack variants. However, our experiment suggests that it is not meaningful to report the size of the attack window as it can be changed in manners described in \lstref{lst:retirement}. However, the speculation window is still limited by the size of the ROB.


\subsection{Speculation Primitive as Prefetchers}
\label{subsec:prefetch}

Some Speculation Primitive may only lead to exploitable vulnerability when the data fetching latency is small---the data is already cached in the L1 cache---but others may succeed even when the data is completely uncached. We speculate the root cause is that some Speculation Primitive, though failed to extract secret from L2, LLC, or memory, could work as a prefetcher to preload secret data into L1 caches so as to facilitate future attacks of the same kind. We empirically validate this hypothesis.

\bheading{Experiments.}
In this test, Windowing Gadget and Disclosure Gadget are unnecessary. The experiment is conducted in three steps: First, the secret data to be accessed by the Speculation Primitive is preloaded (from the shadow virtual address) into the LLC or memory. Second, the tested Speculation Primitive is executed $N$ times (with the exceptions suppressed by the \sysname framework). Third, the data is reloaded from the shadow address and the latency is measured. Two versions of this experiment were tested: (1) $N=0$; (2) $N=1000$.

\bheading{Results.}
When the Meltdown-US variant is selected as the Speculation Primitive, the result of the experiment is shown in \figref{fig:prefetch}. In particular, \figref{fig:prefetch_l3_standard} ($N=0$) and \figref{fig:prefetch_l3_1000} ($N=1000$) show the latency of reloading the secret data that is already in the LLC. %No prefetching is conducted in \figref{fig:prefetch_l3_standard} and prefetching by executing the Speculation Primitive 1000 times is conducted in \figref{fig:prefetch_l3_1000}. 
Clearly with speculative prefetching, the reload latency drops to the range that is close to L2 cache hit. \hl{It suggests that \textit{if the data is already in the LLC, the Speculation Primitive may prefetch it to the L2 cache.}}

\begin{figure}[t]
\centering
\subfloat[Data in LLC, w/o prefetching.]{
    \includegraphics[clip,width=0.47\columnwidth]{fig/prefetch_l3_standard.eps}
    \label{fig:prefetch_l3_standard}
}
\subfloat[Data in LLC, w/ prefetching.]{
    \includegraphics[clip,width=0.47\columnwidth]{fig/prefetch_l3_1000.eps}
    \label{fig:prefetch_l3_1000}
}

\subfloat[Data in memory, w/o prefetching.]{
    \includegraphics[clip,width=0.47\columnwidth]{fig/prefetch_memory_standard.eps}
    \label{fig:prefetch_memory_standard}
}
\subfloat[Data in memory, w/ prefetching.]{
    \includegraphics[clip,width=0.47\columnwidth]{fig/prefetch_memory_1000.eps}
    \label{fig:prefetch_memory_1000}
}

\subfloat[Terminal fault, data in LLC, w/o prefetching.]{
    \includegraphics[clip,width=0.47\columnwidth]{fig/l3_p_standard_prefetch.eps}
    \label{fig:prefetch_l3_standard_present}
}
%\subfloat[From L3, 1 round of attack.]{
%    \includegraphics[clip,width=0.6\columnwidth]{fig/prefetch_l3.eps}
%    \label{fig:prefetch_l3}
%}
\subfloat[Terminal fault, data in LLC, w/ prefetching.]{
    \includegraphics[clip,width=0.47\columnwidth]{fig/l3_p_1000_prefetch.eps}
    \label{fig:prefetch_l3_1000_present}
}
\caption{Reload latency distribution after using Speculation Primitive as a prefetcher.}
\label{fig:prefetch}
\end{figure} 



In addition, if a Disclosure Primitive is used to monitor the covert channel while measuring the reload latency, 1/1000 of the time the correct signal can be received while other times a zero signal is. Because in our previous test we have confirmed that only when data is placed in the L1 cache could it be leaked through speculative execution, \hl{we conclude that \textit{if the data is already in the the L2 cache, the Speculation Primitive has a probability of  prefetching it into the L1 cache.}}

In contrast, in \figref{fig:prefetch_memory_standard} ($N=0$)  and \figref{fig:prefetch_memory_1000} ($N=1000$) , the reload latency distribution does not change with and without prefetching. \hl{Therefore, we can conclude that \textit{if the data is in the memory, the Speculation Primitive cannot prefetch it to the LLC.}}

We conducted another experiment to validate our analysis. This time, the Speculation Primitive accesses a memory page with its \texttt{present} flag cleared. We repeated the experiments with the data originally stored in the LLC. The results are shown in \figref{fig:prefetch_l3_standard_present} ($N=0$) and \figref{fig:prefetch_l3_1000_present} ($N=1000$) . Terminal faults have different prefetching effects. After 1000 rounds of Speculation Primitive execution, although some data is preloaded to L2, the peak still keeps at around 70 cycles (LLC). Only zero signals can be received from the covert channel. 
% According to previous study~\cite{intell1tf}, L1TF attacks leveraging terminal faults can work only when the secret is in L1 cache. 
\hl{\textit{Prefetching with terminal-fault-based attacks is difficult. It is almost impossible to prefetch to L1D.}}

\bheading{Clarifying common misunderstandings of Meltdown-type vulnerabilities.} Since the emergence of the first Meltdown-US paper, one critical question remaining unclear is what exactly are the requirements for a successful attack. The researchers who claimed successful exploitation never released their implementation details. Our study comes to such a claim that \textit{ONE ROUND} of attack is able to correctly fetch the data only when the access latency of the secret is no more than L1D cache latency and the status of TLB has nothing to do with it. And this in fact does not contradict the fact that there are some successful attempts in targeting secret data not in L1D with Meltdown-US. Since the Speculative Primitive of Meltdown-US is able to prefetch inaccessible L2/LLC secret data, a former round of attack is going to facilitate future attacks. Thus, the common description that the attack can steal the non-L1D data but is "slower" is exactly because for slower original caching status, they require more rounds of attack to eventually push the secret into L1D. However, those experiments claiming non-cached secret accessibility do not provide trustworthy proof and may either use other tricks to prefetch secret by the victim itself or leverage other processor internal buffers (whose latency is even lower than L1D cache) as Zombieload~\cite{schwarz2019zombieload}. But these are not the story for L1TF attacks (\eg Foreshadow)~\cite{intell1tf} which require secret to be originally in L1D. Our experiments show that the prefetching effect is unlikely to work properly with terminal faults.
%This is going to be explained in \secref{subsec:prefetch_results}. \yz{TODO: why do we place this paragraph here?}

==> tex/backup-Spectre.tex <==

\subsection{Verifying Misprediction Handling Model}
\label{subsec:misprediction_experiment}

\bheading{Branch misprediction handling.}
As an extended study, the two-phase model also applies to spectre-type misprediction handling. When branch instructions are executed in the back end to determine the branch target address, they leverage the branch prediction units (BPU) to make predictions before the execution completes to improve performance. BPU is a front-end component, making instruction fetching to be immediately redirected to the predicted branch target address. However, if the branch execution unit detects a mismatch between the predicted target address and the true target address, a misprediction is captured by the processor. The misprediction handling is different from exception handling: in \phaseone of misprediction handling, everything required for the handling is performed. The true branch target address is passed to the front end right away once it is determined. All subsequent \uops in ROB are squashed. The IDQ is also flushed. There is no point for the handling to wait until requirement, especially for consideration of performance. % the front end of the execution engine is directly linked to branch execution units, they pass the true target address for instruction fetching right away to the front end and the fetcher is redirected. At the same time, all following instructions in ROB are squashed as in the second phase of exception handling.

\bheading{Test goals.}
Spectre-type branch misprediction attacks is not the subject we focus on in this paper. However, our two-phase model also explains it well but its correctness requires proof by experiments. In addition, the proof is necessary since we leverage this characteristics of branch instructions when implementing some of the suppressing primitives. We need to verify whether the speculative execution is terminated as soon as the prediction is found incorrect, i.e. at \phaseone of the branch instruction, in contrast to at \phasetwo in exception handling.

\begin{lstlisting}[caption={Verifying misprediction handling scheme},label={lst:misprediction}]
// %RAX: address of uncached data
// %RCX: memory address whose data is an address
// to a covert channel buffer

// ---------------------------------------------
// windowing gadget
  [movq (%rax), %rax]
// ---------------------------------------------
// speculation primitive
  branch // poisoned to disclosure gadget
  ...
// ---------------------------------------------
// disclosure gadget
  movq (%rcx), %rcx
  [add $1, %rcx]
  [sub $1, %rcx]
  ...
  movq (%rcx), %rcx
\end{lstlisting}

\bheading{Experiments.}
It is already known that \phasetwo can be delayed by delaying the retirement of the branch instruction. Thus, the key idea of the experiment design is to determine whether the speculative window grows accordingly.

The experiment still follows the \pluginonename design but the speculation primitive is now a branch instruction. Following the sample code in \lstref{lst:misprediction}, we poison the branch instruction to speculatively execute the disclosure gadget. The first speculative instruction in the disclosure gadget loads a value. The last instruction uses this value as the address of a covert channel buffer. Then we try to insert as many ADD/SUB instructions between them as possible for the last instruction to still be executed. The execution of the last instruction is determined using a flush-reload covert channel disclosure primitive. The speculative window is, similar to other experiments, measured by counting the maximal number of permitted ADD/SUB instructions.

The experiment requires a differential analysis. In the first round of the test, no windowing gadget is implemented. In order to slow down the retirement of the branch instruction, we put a slow memory load instruction in the windowing gadget in the second round for comparison. Given different \phasetwo latencies, we observe whether the speculative window are also different.

% \yz{this is not a test per se, this subsection is about a branch instructions as Speculation primitives. How do we integrate this subsection with the others?}




\subsection{Misprediction Handling Model Verification}


Compared to exception handling for meltdown-type attacks, misprediction handling does not involve the idea of exploitability. The only characteristics of interest is the speculation window. During our experiments stated in \secref{subsec:misprediction_experiment}, it is found that the speculation window remains unchanged with or without the slow windowing gadget. This is reasonable since branch prediction is designed for the sake of performance. Squashing the instructions on the wrong path as soon as possible helps speeding up the execution of the instructions on the correct path. Since \phasetwo of the branch instruction has nothing to do with the speculation window, it can only be decided by \phaseone when the true branch target address is resolved. 



==> tex/backup-eval.tex <==
\section{Evaluation}
\label{sec:evaluation}

%In this section, we present the test results of the experiments introduced in \secref{sec:understanding}. As mentioned before, we base most of our analysis on the results of Meltdown-US \cite{Lipp2018meltdown} as it is a most typical example. It will be pointed out when results are found different with other variants.

\subsection{Understanding Two Phase Model}

To establish the relationship between the two-phase model and the \textit{exploitability} and \textit{attack window} of the \vulname vulnerabilities, we run tests to understand the effects of \phaseone and \phasetwo of a Speculation Primitive. A variant of Meltdown is used as the Speculation Primitive. The experiments were conducted on an Intel i7-7700HQ machine with Ubuntu 16.04 (Linux 4.4.0-137) as the operating system. It is found that the conclusions made from the experiments are also true on all other tested processors. %, since we abstract implementation-specific details in the two-phase model as explained in \secref{subsec:handling}. 
On the sample machine, each experiment is repeated for 5 times for reliability.

\subsubsection{Effect of \phasetwo}
\label{subsec:e2_effect_eval}

In the experiment described in \secref{subsec:e2_effect}, we observed that when the inserted instructions exceed a threshold, the covert-channel receiver no longer receive any signal from the covert channel. As the number is much smaller than the size of ROB \cite{measuring-rob}, it is not cause by ROB limits. As a conclusion, \textit{issued instructions will be squashed due to an exception at \phasetwo. Any instruction not yet executed will not be executed at all.}
\yx{added a sentence} In other words, \phasetwo determines the "attack window" for the secret to be transferred by covert channel.

\subsubsection{Effects of \phaseone}
\label{subsec:e1_existence_eval}

In the experiment described in \secref{subsec:e1_existence}, we observe that only when the secret data is stored in the L1 cache can the correct covert-channel signal be received. When the secret data is store in L2, LLC, or the memory, a zero signal is received. This observation validates our theory in \ref{subsec:handling}. The execution unit stops execution after catching the exception; a dummy value of zero is returned as the result of the execution. This process is what we define as \phaseone. Therefore, this experiment concludes that \textit{(1) \phaseone makes the execution result to be zero, without squashing the execution. (2) If the latency of \phaseone is later than the data fetching latency, the correct value can be propagated to the speculative instructions; otherwise, a zero value will be used instead.}

%Combining the results to be shown in \secref{subsec:e2_change_eval} proving the data fetched has nothing to do with \phasetwo, we are confident to conclude the existence of \phaseone which stops the execution unit that triggers the exception.
% The other finding is that the attack window is always fixed regardless of the memory access latency. However, we are still unable to conclude the relationship between disclosure gadget squash and the two phases since the latency of either is fixed. Further studies are explained in the following parts.

In both experiments described in \secref{subsec:e1_effect}, regardless of whether the two Speculation Primitives accesses the same memory addresses or not, by gradually inserting instructions between them, we never witnessed that the received covert-channel signal changes from the correct value to zero. Instead, we only observed that after some threshold, the signal disappears. To conclude,\textit{ \phaseone of the first Speculation Primitive does not affect other execution units.} This also means there is no need to specially consider attacks that place two Speculation Primitives together.

%the latency of the second speculation primitive is gradually changed by inserting ADD/SUB instructions one by one as stated in \secref{subsec:e1_effect}. We never witness the covert channel buffer corresponding to 0 being touched when the two speculation primitives access the same address.

%When the two speculation primitives access different addresses, we try setting the data of the first address to be in either L1D or L2 cache. It is known by \secref{subsec:e1_existence_eval} that L1D latency is shorter than \phaseone latency while L2 latency is longer. However, in both experiment settings, the data could still either be correctly used as 0x42000 or not used at all. To conclude, \phaseone of the first speculation primitive only kills the execution on its own execution unit without influencing any other execution units in the execution component of the execution engine.


In the experiment described in \secref{subsec:e1_exec}, when changing the TLB status of the page storing the secret data, \phaseone latency is also altered. However, we did not observe any changes in the speculation window. Therefore, we conclude that \textit{\phaseone has no influence on the entire execution engine}.

\yx{added a paragraph}
Since the emergence of the first Meltdown-US paper, one critical question remaining unclear is what exactly are the requirements for a successful attack. Our study provides such a claim that \textit{ONE ROUND} of attack is able to correctly fetch the data only when the secret is in L1D cache and the status of TLB has nothing to do with it. And this in fact does not contradict the fact that there are some successful attempts in targeting secret data not in L1D. This is going to be explained in \secref{subsec:prefetch_results}.

%The first experiment focuses on the effect of \phaseone on other components of the execution engine by seeing whether the speculation window changes when we change the TLB availability as the discovery of exception has to wait for TLB entry to be available. However, during experiments, we do not see any change in the speculation window. Thus, \phaseone has no influence on the squashing of speculative instructions.



\subsection{Measuring \vulname Vulnerability}

We performed tests on 9 machines and the test results are provided in Table \ref{tbl:exploitability}. The test machines include 2 laptops, 5 desktops and 1 cloud VM. All tested machines run Ubuntu 16.04 with Linux kernel 4.4.0-137 (or 4.4.0-141 for compatibility issues on newer hardware) and KPTI is turned off. KPTI as a software patch may make our study on the PTE-US variant inaccurate.

All the Intel microcode versions are rolled back to version 20171117 to make sure later microcode patch does not influence our tests. The only two exceptions are with Coffee Lake (no old microcode) and cloud VM (no control over microcode). But the tests on these two machines also show no influence by the microcode patch. The AMD microcode version is 3.20180515.1.
\yx{added something here}
We do not test all machines with up-to-date microcode patch because the core of our study is to understand the true nature of transient execution attacks systematically on hardware level. The tool may also be useful in verifying the effectiveness of patches, but this is not within the scope of this paper.

\subsubsection{Exploitability}

\begin{table*}[tb]
\begin{center}
{\scriptsize
\begin{tabular}{p{0.35\columnwidth}|p{0.13\columnwidth}|p{0.13\columnwidth}| p{0.14\columnwidth}|p{0.14\columnwidth}|p{0.16\columnwidth}|p{0.13\columnwidth}|p{0.12\columnwidth}|p{0.15\columnwidth}|p{0.13\columnwidth}}
 & Laptop 1 & Laptop 2 & Desktop 1 & 
Desktop 2 & Desktop 3 & Desktop 4 & Desktop 5 & Desktop 6 & Cloud 1 \\ 
Variant & KabyLake & KabyLake & Haswell-EP & SandyBridge & Westmere-EP & CoffeeLake & KabyLake & AMD EPYC & Skylake-SP \\
\toprule

PTE (Present) & Y & N/A & N/A & N/A & N/A & Y & Y & N/A & Y \\ \hline

PTE (Reserved) & Y & N/A & N/A & N/A & N/A & Y & Y & N/A & Y \\ \hline

PTE (US) & Y & Y & Y & Y & Y & Y & Y & R & Y \\ \hline

Load CR4 & R & R & R & R & R & R & R & R & R \\ \hline

Load MSR (0x1a2) & R & R & R & R & R & R & R & N/A & N/A \\ \hline

Protection Key (User) & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & Y \\ \hline

Protection Key (Kernel) & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & Y \\ \hline

SMAP violation & Y & Y & N/A & N/A & N/A & Y & Y & Y* & Y** \\ \hline

PTE (write w/ RW=0) & Y & Y* & Y & Y & Y & Y & Y & R & Y \\ \hline

Load xmm0 (CR0.TS) & Y & Y & Y & Y & Y & Y & Y & N/A & N/A \\ \hline

BOUND (32-bit) & Y & Y & Y & Y & Y & Y & Y & Y & Y \\ \hline

DS Over-Limit (32-bit) & N & N & N & N & N & N & N & Y & N \\ \hline

SS Over-Limit (32-bit) & N & N & N & N & N & N & N & Y & N/A \\ \hline

DS Not-Present (32-bit) & R & R & R & R & R & R & R & R & R \\ \hline

SS Not-Present (32-bit) & R & R & R & R & R & R & R & R & R \\ \hline

DS Execute-Only (32-bit) & R & R & R & R & R & R & R & R & R \\ \hline

CS Execute-Only (32-bit) & R & R & R & R & R & R & R & R & R \\ \hline

DS Read-Only (write, 32-bit) & Y & Y & Y & Y & Y & Y & Y & R & Y \\ \hline

SS Read-Only (32-bit) & R & R & R & R & R & R & R & R & R \\ \hline

DS Null (32-bit) & N & N & N & N & N & N & N & R & N \\ \hline

SS Null (32-bit) & R & R & R & R & R & R & R & R & R \\ \hline

SS $DPL \neq CPL$ (32-bit) & R & R & R & R & R & R & R & R & R

\end{tabular}
}
\end{center}
\vspace{-10pt}
\caption{Exploitability evaluation on different machines. Y: exploitable. N: non-exploitable. R: no speculative execution. N/A: unable to test. Y*: both expected data and zero data are captured in all covert channel reloads. Y**: the only exploited case with success rate not 100\% (about 60\%). Laptop 1: i7-7820HQ (Kaby Lake). Laptop 2: i7-7700HQ (Kaby Lake). Desktop 1: Xeon E5-1607v3 (Haswell-EP). Desktop 2: i3-2120 (Sandy Bridge). Desktop 3: Xeon E5620 (Westmere-EP). Desktop 4: Xeon E-2124G (Coffee Lake). Desktop 5: i7-7700 (Kaby Lake). Cloud 1: Amazon EC2 C5 instance. Desktop 6: AMD EPYC 7251.}
\label{tbl:exploitability}
\end{table*}

In this section, we systematically test whether a certain candidate variant is exploitable by measuring whether \phaseone latency is longer than data fetching latency. The tested variants are enumerated from the exception list we explain in \secref{subsec:instruction_model}. The results are shown in \tabref{tbl:exploitability} and a reference of the tested variant names to their description can be found in \secref{sec:exception_list}. Some variants are unable to be tested due to lack of hardware support or OS support on certain machines and they are marked as N/A. On the tested Intel machines, Meltdown-US (accessing supervisor memory page from user space) and Meltdown-RW (writing to a read-only memory page) are exploitable while the AMD machine shows no speculation. When testing Meltdown-Present (\texttt{Present} flag cleared) and Meltdown-Reserved (\texttt{Reserved} flag set), signal handler cannot be used since the whole OS will crash. Thus, only the machines also equipped with Intel TSX~\cite{inteltsx} are tested and reported. Loading restricted registers (CR4 and MSR) on all tested machines show that no speculative load is allowed. Meltdown-MPK (bypassing the restriction of memory protection keys) could only be tested on Amazon EC2 E5 instance and it was found exploitable. Meltdown-FP (accessing a lazy-context-switch float pointer register) is also found exploitable on Intel machines. Meltdown-BR ( accessing an array with an over-range index) is found exploitable on all tested machines although the BOUND instruction raises an exception when it discovers the violation. In 32-bit mode, segmentation is enabled and thus relevant variants could be tested. Most of them are not exploitable or does not allow further speculation at all, since paging checks has to wait until segmentation translation produces a linear address while segmentation check begins at the same time as the translation. However, still some of them are found exploitable on either Intel or AMD platform.

%One new variant on this basis is discovered and will be explained shortly. Meltdown-SMAP, also a newly found variant, is possible to be expoited on all testable platforms and we will explain it in more details. 



%We find that among the 100,000 rounds of repeated tests in all tested variants, at most one of the covert channel buffer entries could be touched. And when one of them (either corresponding to the correct data or to zero) shows a hit, the hit rate is above 99\%.

In our experiments, a few new variants were found by the \sysname framework. \textit{We have reported these new variants to Intel and AMD already.}

\bheading{Supervisor mode access violating SMAP (Intel \& AMD).}
Supervisor Mode Access Prevention (SMAP) forbids code in the kernel mode from accessing to user-space addresses.  However, as shown in \tabref{tbl:exploitability}, on some of our tested machines, SMAP can be bypassed using speculative execution when the secret data is in the L1 cache. When the data is in lower-level caches, zero signal is captured. %In fact, for all the new and known exploitable cases with the one-load-instruction model, we found that they were exploitable only when the secret data was in L1 cache. Presence of TLB entry does not influence exploitability in the case of SMAP. 

\bheading{Supervisor mode access bypassing MPK (Intel).}
When a user space page is set to be inaccessible using Memory Protection Key (MPK), its accesses from kernel code is also forbidden, which triggers a page fault exception. However, as demonstrated on the tested cloud server (see \tabref{tbl:exploitability}), if the secret data is already in the L1 cache, it can be leaked through speculatively executed Disclosure Gadget. 

\bheading{Memory write to read-only data segments (Intel).}
Segmentation is used in the 32-bit mode. However, memory write to a read-only data segments can be speculatively  speculatively used by following instructions. In this case, the caching and TLB status does not affect the exploitability. This vulnerability is similar to the \texttt{Meltdown-RW}, but its security implication is different: \texttt{Meltdown-RW} takes advantage of store-to-load forwarding. As the store buffer is indexed by the linear address (not virtual address), the forwarding is speculative as the logical-to-physical translation is not yet finished. Therefore, it is not surprising that the permission check (using flags in the PTE) happens after the store-to-load forwarding. However, in contrast, the segmentation check is performed during the translation from logical addresses to linear addresses. Thus, when the store buffer queues the store instruction to the given logical address \cite{US6378062}, the segmentation access privilege check should already be done. However, surprisingly, our test suggests that this is not the case as a following load could directly use the store value.

%which is indexed by linear addresses to increase performance by temporarily ignoring physical address translation through paging. Thus, when such forwarding happens speculatively, it is not surprising that the checking of page table access privileges is still pending since it has to wait until the physical address translation completes to get corresponding flags in page structre entries. In contrast, segmentation check is performed during the translation from logical addresses to linear addresses. Thus, when the store buffer queues the store instruction to the given logical address \cite{US6378062}, the segmentation access privilege check should already be done. 
% \yx{US patent 6378062 (Intel) description:Once the linear address is calculated, it is stored in the store address buffer (SAB).} 

%In this case, the caching and TLB status does not affect the exploitability. 

\bheading{Reading from a logical address over the limit of segment (AMD).}
When testing in 32-bit mode, a load to a logical address beyond the segment limit is forbidden, which triggers an exception. However, we have found that the segmentation check can be bypassed by speculative execution. The vulnerability is exploitable when the TLB entry of the page is present and the data is cached in the L1 cache. The same vulnerability cannot be found in Intel processors.

%This variant is most similar to the original Meltdown but the threat model is slightly different. The variant is not intended to access memory in another address space but to break the access limit enforced by segmentation within the address space of the process. Such variant is found not applicable to Intel processors.



\subsection{Quantitative Measurement of \phaseone Latency}
\label{subsec:e1_change_eval}

%To understand the controllability over \phaseone, we need to quantitatively measure this micro-architecure state. The tests proposed in \secref{subsec:e1_change} provide a novel method to carry out the measurement, but it has some limitation. To be tested by the method, the test cases need to satisfy two conditions. First, the test case must conform to the one-load-instruction model discussed in \secref{subsec:instruction_model}, since we are measuring the latency for loading zero value to substitute directly measuring exception capturing latency, which is architecturally invisible. Second, the speculation primitive in the test case must allow speculative execution. In other words, it must be tested as either "exploitable" or "in-exploitable" by \secref{subsec:e1_measure}. 

For the tests that yield $Y$ or $N$ in \tabref{tbl:exploitability}, further analysis can be conducted in test described in \secref{subsec:e1_change}. The only exception happens when the exception is triggered by a \texttt{reserved} flag set or a \texttt{present} flag cleared. In these two cases, although they were found "exploitable", when tested using \lstref{lst:framework2}, no covert-channel signal can be received. This is because these page faults are terminal terminal faults, which are treated differently under speculative execution. 

%Among our test cases, there are two special cases meeting the requirements but are unable to be tested. When a reserved bit is set or the present bit is cleared in the page table entry, the page fault triggered is a terminal fault. During our experiments, we found that when trying to suppress such terminal faults using any of the proposed methods, the covert channel access instruction is unable to receive any data from the speculation primitive, although they are both found "exploitable" by the first framework.

% \begin{figure*}[t]
% \centering
% \subfloat[\phaseone measurement with exception-based suppression.]{
%     \includegraphics[clip,width=0.95\columnwidth]{fig/option2_exception_.eps}
%     \label{fig:p1_exception}
% }
% \subfloat[\phaseone measurement with retpoline-based suppression]{
%     \includegraphics[clip,width=0.95\columnwidth]{fig/option3_retpoline_.eps}
%     \label{fig:p1_retpoline}
% }
% \caption{Comparison between different suppression methods in the implementation of \phaseone measurement framework.}
% \end{figure*}
% \label{fig:suppression}

\begin{figure*}[t]
\minipage{0.7\textwidth}
    \subfloat[Exception-based suppression.]{
        \includegraphics[clip,width=0.47\linewidth]{fig/option2_exception_.eps}
        \label{fig:p1_exception}
    }
    %\hfill
    \subfloat[Retpoline-based suppression]{
        \includegraphics[clip,width=0.47\linewidth]{fig/option3_retpoline_.eps}
        \label{fig:p1_retpoline}
    }
    \caption{Comparison between different suppression methods.}
\endminipage\hfill
\minipage{0.28\textwidth}%
    \includegraphics[width=\linewidth]{fig/atk_window_xmm_.eps}
    \caption{Size of the effective Windowing Gadget vs. speculation windows.}
    \label{fig:atk_window_xmm}
\endminipage
\vspace{-11pt}
\end{figure*}


\subsubsection{Choosing The Best Suppressing Primitive} We explore two implementations of the Suppressing Primitive: exception-based and retpoline-based. An exception-based Suppressing Primitive is illustrated in \lstref{lst:framework2}. The other uses a retpoline to suppress exceptions~\cite{stecklina2018lazyfp}. We evaluated these methods using the following method: 
Using each method, we gradually insert ADD/SUB instructions to find the maximum speculation window. The covert-channel tests were repeated 100,000 times for each number of inserted instructions. The rate of receiving the covert-channel signals for each number is illustrated in  \figref{fig:p1_exception} and \figref{fig:p1_retpoline}, respectively. It can be seen from the figures that the retpoline-based approach is less desirable as the rate of receiving the signal drops gradually when the inserted instructions increases, making it hard to determine the speculation window. Therefore, in our test, the exception-based approach is used.

%With a given suppressing primitive, we still need to repeat the test with a given number of inserted ADD/SUB instructions for 100,000 times. And by counting the hit rate we decide whether the covert channel instruction is executed. This ensures reliability but also leads to a problem of hit rate threshold. When suppressing the tested speculation primitive with another exception, we could clearly see the hit rate is either above 90\% or less than 10\%, as shown in \figref{fig:p1_exception}, thus solving the threshold issue naturally. When trying the other methods, the hit rate number corresponding to the number of inserted instructions drop gradually as demonstrated in \figref{fig:p1_retpoline}, making it hard to determine a reasonable threshold. As a result, all following tests in this section are performed with the exception-based suppressing primitive as shown in the code sample in Listing \ref{lst:framework2}.

%In this section, we demonstrate two sample case studies with the proposed experiment to analyze the \phaseone latency. They are two typical examples and the results are found also true for other similar variants.

\subsubsection{Quantitative Analysis}

The test described in \lstref{lst:framework2} enables quantitative analysis of the vulnerability. It helps us explain why some vulnerabilities are exploitable and others are not. For instance, when the Speculation Primitive is a kernel memory read from userspace, the L1 data fetching latency is smaller than the latency of \phaseone, so the correct value can be leaked. Moreover, the results of the test suggest $T_{data} - T_{P1} = 0$, which means \phaseone and L1 cache data fetching arrives at the same cycle. This also explains why the attack cannot work when the data is in higher-level caches, confirming our conclusion in \secref{subsec:e1_existence_eval}. 
\yx{added a sentence here} The data further answer the common question of why Meltdown-US attacks often capture zeros as the results. In real-world attack settings with no intentional interference, the likelihood for the secret data to be in L1D is much lower than in L2, LLC or memory.

%For the differential analysis, we pick two execution environments that respectively yield expected data and zero data. In both environments, the US flag of the page table entry is set. The first execution environment forces the data to be in L1 while the second one flushed to memory. In both cases, the TLB entry is flushed. We found that the maximal number of inserted ADD/SUB instructions that still allows the last covert channel access instruction to execution are the same for both cases. As a result, the exception capturing latency is in fact the same as the L1 data fetching latency, yielding a zero relative latency. So the race between them is just in time for the attacker. 


The test also enables analysis of negative results in \tabref{tbl:exploitability}. For example, when accessing data beyond the segment limit, data in \tabref{tbl:exploitability} suggest the vulnerability is not exploitable. By running the test to quantitatively measure $T_{P1}$, we were surprised by find out that $T_{data} - T_{P1} = 0$, which means \phaseone come right before the data is available.  
However, when data is available in the L2 cache, we find $T_{data} - T_{P1} = -12$, which suggests \phaseone come 12 cycles earlier than the data is available.



%Negative results here refer to the experiments marked $N$ (non-exploitable). It is desireable to investigate the negative results further so as to make conclusive assertions. Here we illustrate our analysis using the \texttt{Meltdown-Segment} example.

%In order to carry out differential analysis, we still need two execution environments that respectively yield expected data and zero data. Thus, for the first environment we set the limit of the segment descriptor to be greater than the accessed address while for the second less. Both of them force the data in L1D cache and the TLB entry present. The test result suggests that the difference of maximal number of inserted ADD/SUB instructions between these two cases is also zero. That is to say, the race between segmentation check and data fetching from L1D cache just fails even when in best scenario.


%One thing to point out here is that the L1 latency is different from what we can measure using RDTSC(P) instruction. It is the latency from the beginning of execution to when the data value could be speculatively used by following instructions.


%There is always a doubt of whether the failure of the attack is really due to the nature of the variant itself or simply bad attack design, and we are able to answer it by seeing the true architectural status of the execution using the proposed tool. We provide the in-exploitable case of trying to read an over-segment-limit logical address as an example and analyze the changeability of \phaseone with such variants.


\subsubsection{Changing \phaseone Latency}

The test described in \lstref{lst:framework2} also enable us to reason about whether \phaseone of a Speculation Primitive can be delayed by changing the instruction sequences. This is critical as it matters to whether the exploitability of a vulnerability can be manipulated by software.

In the Speculation Primitives that involves exceptions raised by permission checks in PTEs, the absolute \phaseone latency (execution of the instruction to \phaseone) includes two components: TLB entry loading and permission checking. Similarly, the absolute latency of data fetching (execution of the instruction to data ready) also includes two components: TLB entry loading and data fetching. Therefore, the relative \phaseone latency (data available to \phaseone) only depends on the latency of permission checking and that of data fetching, both of which happens after the TLB entry is ready. Therefore, by altering TLB status, the relative \phaseone latency cannot be changed. We have verified this discussion in the test described in \lstref{lst:framework2}. When keeping the cache status of the secret data unchanged, it is found that the relative \phaseone latency remains the same in the experiments.

%Meanwhile, as the data fetching also begins right after the TLB entry becomes available, the absolute latency of data fetching (TLB ready to data ready) is also fixed, if the data is available in L1. Therefore, the relative latency of \phaseone (data available to \phaseone) cannot be altered in this case. 

In the Speculation Primitives that involves exceptions raised by other checks, however, the relative \phaseone latency can be changed. For example, when the exception is raised by segmentation fault, the absolute \phaseone latency has nothing to do with TLB loading, because the exception is raised before page-level checking; however, the data fetching latency can be delayed by flushing TLBs. Therefore, the relative latency of \phaseone can be decreased by TLB preloading. Therefore, the optimal attack is represented by the condition with TLB entries present and secret data in the L1 cache. If in the optimal attack, the data fetching fails to outrun \phaseone, the vulnerability is not exploitable. In the experiment, flushing the TLB entries (compared to preloading them) leads to a decrease of the relative \phaseone latency of over 100 cycles.


%When flushing the TLB entry but keeping the data in L1D, the difference between the two cases becomes greater than 100. But thus it is hard to get the exact number due to ROB size limit as explained before. However, it is already clear that TLB status does influence the race between exception capturing and data fetching a lot. But even when TLB entry is present, the attacker is still unable to win. Another conclusion we could make is that the \phaseone latency here is not influenced by either caching or TLB status. This is reasonable since the checking of limit happens during segmentation translation, before paging translation. According to our two-phase exception handling model, as soon as the CPU notices an access violation (at \phaseone), the instruction execution immediately stops and provides a dummy zero as the data fetching result. This well explains the experiment results we get from our tool framework.





\subsection{Measuring and Changing \phasetwo Latency}
\label{subsec:e2_change_eval}



% \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{fig/atk_window_xmm_.eps}
% \caption{Relationship between the length of windowing gadget (X-axis) and attack window (Y-axis).}
% \label{fig:atk_window_xmm}
% \end{figure}

In \figref{fig:atk_window_xmm}, the x-axis is the effective size of Windowing Gadget (tuned by moving the position of CPUID) and the y-axis is speculation window. By gradually moving the position of CPUID from the beginning of the Windowing Gadget to the end, which changes the effective length of windowing gadget, the speculation window also grows accordingly. Therefore, we conclude that \textit{\phasetwo latency can be increased}. Prior studies~\cite{Lipp2018meltdown} have reported the attack window of certain attack variants. However, our experiment suggests that it is not meaningful to report the size of the attack window as it can be changed in manners described in \lstref{lst:retirement}. However, the speculation window is still limited by the size of the ROB.

%To make the conclusion more convincing, we we need to verify that the retirement of the speculation primitive is correctly delayed with IACA. IACA analysis shows that the speculation primitive could always be executed shortly after it is issued. On the meanwhile, with longer windowing gadget, its retirement is more delayed. Combining the two facts demonstrated above, we are confident to conclude that squashing of the speculative instructions is performed at \phasetwo.

%What's more, when we force the data fetching latency and \phaseone latency to be constant, the data fetched by the speculation primitive does not change (either the correct value or zero as stated in \secref{subsec:e1_existence}) no matter how \phasetwo latency changes. Thus, the data fetching execution is not relevant to \phasetwo.



\subsection{Speculation Primitive as a Prefetcher}
\label{subsec:prefetch_results}

%To answer the interesting question of whether the previous round of attack could help the next round, we look into whether the speculation primitive is able to push inaccessible data into cache as a prefetcher. Experiment design is presented in \secref{subsec:prefetch}.

\begin{figure}[t]
\centering
\subfloat[Data in LLC, w/o prefetching.]{
    \includegraphics[clip,width=0.47\columnwidth]{fig/prefetch_l3_standard.eps}
    \label{fig:prefetch_l3_standard}
}
\subfloat[Data in LLC, w/ prefetching.]{
    \includegraphics[clip,width=0.47\columnwidth]{fig/prefetch_l3_1000.eps}
    \label{fig:prefetch_l3_1000}
}

\subfloat[Data in memory, w/o prefetching.]{
    \includegraphics[clip,width=0.47\columnwidth]{fig/prefetch_memory_standard.eps}
    \label{fig:prefetch_memory_standard}
}
\subfloat[Data in memory, w/ prefetching.]{
    \includegraphics[clip,width=0.47\columnwidth]{fig/prefetch_memory_1000.eps}
    \label{fig:prefetch_memory_1000}
}

\subfloat[Terminal fault, data in LLC, w/o prefetching.]{
    \includegraphics[clip,width=0.47\columnwidth]{fig/l3_p_standard_prefetch.eps}
    \label{fig:prefetch_l3_standard_present}
}
%\subfloat[From L3, 1 round of attack.]{
%    \includegraphics[clip,width=0.6\columnwidth]{fig/prefetch_l3.eps}
%    \label{fig:prefetch_l3}
%}
\subfloat[Terminal fault, data in LLC, w/ prefetching.]{
    \includegraphics[clip,width=0.47\columnwidth]{fig/l3_p_1000_prefetch.eps}
    \label{fig:prefetch_l3_1000_present}
}
\caption{Reload latency distribution after using Speculation Primitive as a prefetcher.}
\label{fig:prefetch}
\end{figure} 

When the original Meltdown variant is selected as the Speculation Primitive, the results of the experiment described in \secref{subsec:prefetch} is shown in \figref{fig:prefetch}. In particular, \figref{fig:prefetch_l3_standard} and \figref{fig:prefetch_l3_1000} show the latency of reloading the secret data that is already in the LLC. No prefetching is conducted in \figref{fig:prefetch_l3_standard} and prefetching by executing the Speculation Primitive 1000 times is conducted in \figref{fig:prefetch_l3_1000}. Clearly with speculative prefetching, the reload latency drops to the range that is close to L2 cache hit. It suggests that \textit{if the data is already in the LLC, the Speculation Primitive may prefetch it to the L2 cache.} 

In addition, if a Disclosure Primitive is used to monitor the covert channel while measuring the reload latency, 1/1000 of the time the correct signal can be received while other times a zero signal is. Because in our previous test we have confirmed that only when data is placed in the L1 cache could it be leaked through speculative execution, we conclude that \textit{if the data is already in the the L2 cache, the Speculation Primitive has a probability of  prefetching it into the L1 cache.}

%Compared to the fact that one single execution of the Speculation Primitive with data originally in L3 cache could never fetch the correct data, it could be concluded that repeated execution of the Speculation Primitive has a chance of prefetching secret even to L1 cache.

In contrast, in \figref{fig:prefetch_memory_standard} and \figref{fig:prefetch_memory_1000}, the reload latency distribution does not change with and without prefetching. Therefore, we can conclude that \textit{if the data is in the memory, the Speculation Primitive cannot prefetch it to the LLC.}

We conducted another experiment to validate our analysis. This time, the Speculation Primitive accesses a memory page with its \texttt{present} flag cleared. We repeated the experiments with the data originally stored in the LLC. The results are shown in \figref{fig:prefetch_l3_standard_present} and \figref{fig:prefetch_l3_1000_present}. Terminal faults have different prefetching effects. After 1000 rounds of Speculation Primitive execution, although some data is preloaded to L2, the peak still keeps at around 70 cycles (LLC). Only zero signals can be received from the covert channel. %And the data fetched is found to be almost all zero, with only around 3 in a million shown to be the correct value. However, such a low probability is more like noise from the covert channel. 
According to previous study~\cite{intell1tf}, L1TF attacks leveraging terminal faults can work only when the secret is in L1 cache. This is likely due to the difficulty of the prefetching with terminal-fault-based attacks.

%In the figures of LLC experiment, we could see the reload latency tends to be shorter after one faulty access while most reload latency turns out to be from L2 after 1000 faulty accesses. The experiments on data originally in L2 have a problem with RDTSCP timing accuracy so in these experiments L2 latency cannot be well distinguished from L1 latency. However, we could see when the data is originally in memory, the likelihood of it being pushed to memory seems to be zero. The phenomenon are reasonable in that the data fetching from higher level to lower, if not finished, will be ceased by exception handling phase one. Within the limited time, the slow memory load into memory is unlikely to complete while L3 data is more likely to be pushed to L2.





==> tex/backup-exception.tex <==
\begin{itemize}
\item Page-fault exceptions (\#PF).

Notice that entries from TLB, paging-structure caches or paging structures in memory (privilege from higher to lower) may have different effects.

(1) No translation for the virtual address.
\begin{itemize}
\item P flag is set in any paging-structure entry.
\item Any of the reserved bits are set in any paging-structure entry.
\end{itemize}

(2) Access rights violation.

One point to notice in below rules is that protection key is only effective when CR4.PKE = 1 with IA-32e paging. Rules (defined in PKRU register) for protection key i of a user-mode address are: if AD(r) = 1, no data accesses are permitted; if WD(r) = 1, supervisor-mode writes with CR0.WP = 1 or user-mode writes are not permitted.

\begin{itemize}
\item Supervisor-mode accesses.

(r) Data reads from/writes to user-mode addresses.
\begin{itemize}
\item CR4.SMAP = 0 AND no permitting protection key*.
\item CR4.SMAP = 1 AND (EFLAGS.AC = 0 OR the access is implicit).
\item CR4.SMAP = 1 AND (EFLAGS.AC = 1 AND no permitting protection key*).
\end{itemize}

(ii) Data writes to supervisor-mode/user-mode addresses. 
\begin{itemize}
\item CR0.WP = 1 AND R/W flag is 0 in any paging-structure entry.
\end{itemize}

(iii) Instruction fetches from supervisor-mode addresses.
\begin{itemize}
\item (PAE paging OR IA-32e paging with IA32\_EFER.NXE = 1) AND XD flag is 1 in any paging-structure entry.
\end{itemize}

(iv) Instruction fetches from user-mode addresses.
\begin{itemize}
\item CR4.SMEP = 1.
\item CR4.SMEP = 0 AND (PAE paging OR IA-32e paging with IA32\_EFER.NXE = 1) AND XD flag is 1 in any paging-structure entry.
\end{itemize}
\end{itemize}

\begin{itemize}
\item User-mode accesses

(r) Data reads.
\begin{itemize}
\item No permitting protection key*.
\item From supervisor-mode addresses.
\end{itemize}

(ii) Data writes.
\begin{itemize}
\item R/W flag is 0 in any paging-structure entry.
\item No permitting protection key*.
\item To supervisor-mode addresses.
\end{itemize}

(iii) Instruction fetches.
\begin{itemize}
\item (PAE paging OR IA-32e paging with IA32\_EFER.NXE = 1) AND XD flag is 1 in any paging-structure entry.
\item From supervisor-mode addresses.
\end{itemize}

\end{itemize}

(3) SGX-induced page fault.

\begin{itemize}
\item Enclave accesses to enclave pages via illegal virtual addresses.
Enclave accesses to PT\_REG, PT\_TCS or PT\_TRIM enclave pages use virtual addresses other than the ones that the pages are originally mapped to within ELRANGE during allocation.

\item Direct Enclave Accesses to EPC pages causing EPCM security attributes violation.

(r) Target page does not belong to current enclave.

(ii) Writes to pages denied write access by EPCM.

(iii) Reads to pages denied read access by EPCM.

(iv) Instruction fetches to pages denied execute access by EPCM.

(v) Target page has a restricted page type, i.e. PT\_SECS, PT\_TCS, PT\_VA, or PT\_TRIM.

(vi) The target page is in BLOCKED, PENDING or MODIFIED state.

\item Special case triggering non-SGX-induced page faults related to implicit enclave access.
When physical addresses used by implicit enclave access instructions are cached, they may also trigger exceptions (or VM exits) during checks such as segmentation, paging, EPT, and APIC virtualization checks.

\end{itemize}

\end{itemize}

\begin{itemize}
    \item General protection (\#GP)

    (1) SGX mode code fetches.
    \begin{itemize}
        \item From inside an evclave to virtual addresses outside enclave.
        \item Splitting across ELRANGE from inside an evclave.
    \end{itemize}
    
    (2) Instruction length limit exceeded.
    Caused by redundant instruction prefixes.
    
    (3) Loading CR0 with PG = 1 AND PE = 0.
    
    (4) Loading CR0 with NW = 1 AND CD = 0.
    
    (5) Write 1 to a reserved bit of CR4.
    
    (6) Executing a privileged instruction from non-privileged mode (CPL $\neq$ 0).
    Privileged instructions include: LGDT, LLDT, LTR, LIDT, MOV CR\#, LMSW, CLTS, MOV (debug registers), INVD, WBINVD, INVLPG, HLT, RDMSR, WRMSR, RDPMC, PDTSC.
    
    (7) Writing 1 to a reserved bit of MSR.
    
    (8) Any reserved bit set to 1 in PDPT entry AND (CR4.PAE = 1 AND/OR CR4.PSE = 1).
    Checked when reloading PDPT due to writes to CR0, CR3 or CR4.
    
    (9) Write 1 to a reserved bit of MXCSR.
    
    (10) Accessing a 128-bit memory location not aligned when executing a SSE/SSE2/SSE3 instruction.

\end{itemize}

\begin{itemize}
    \item Divide Error Exception (\#DE)
    \yx{Do we include this?}
\end{itemize}

\begin{itemize}
    \item Debug Exception (\#DB)
    \yx{Do we include this?}
\end{itemize}

\begin{itemize}
    \item Invalid Opcode Exception (\#UD)
    \yx{Do we include this?}
\end{itemize}

\begin{itemize}
    \item Device Not Available Exception (\#NM)
    \yx{Do we include this?}
\end{itemize}

\begin{itemize}
    \item Stack Fault Exception (\#SS)
    (1) Limit violation.
    Could be caused by POP, PUSH and memory reference instructions using SS register explicitely or implicitely.
    
    (2) Non-present stack segment.
    Could be caused by a MOV or POP instruction to the SS register. Other causes are not relevant to memory access.
    
    (3) Canonical violation.
    Caused by accessing memory using SP register that contains a non-canonical address in 64-bit mode.
\end{itemize}

And below lists non-exceptional protections:

\begin{itemize}
\item Accesses to SGX enclave

(1) Non-enclave accesses to EPC memory result in altered behavior.

(2) A data access that splits across ELRANGE from inside an enclave is separated by processor into two data accesses and each access is evaluated.

\end{itemize}

==> tex/backup-fuzzer.tex <==
\section{Fuzzer Design}
\label{sec:experiments}

The fuzzer model is made up of an instruction sequence and an execution environment. The instruction sequence includes three major parts: preceding instructions, faulty instruction and speculative instructions for attack window measurement. \yx{Two faulty instructions not tested yet.} If preceding instructions are found not related to the speculative execution of the faulty instruction, there is no need to worry about them. As for the second part, the method to generate a faulty instruction is elaborated in \ref{subsubsec:instruction_model}. It involves not only an instruction, but also conditions such as page tables. When measuring the attack windows, positive attack windows could be directly exposed by covert-channel based method. But when the window is negative, we need to measure exception handling latency and data available latency separately.

\subsection{Overview}
\label{subsec:experiment_overview}

\yx{Keep this subsec?}

\textbf{Attack window measurement.}
Given the fact that some conditions for a greatest possible exception handling latency may conflict with those for a short or minimal data load latency, we need additional experiments to the real attack window in different conditions and find the maximal possible settings.

We take into account several factors that influence the attack window. First is the load latency of the secret. The secret may lie in L1, L2, LLC or memory. Although it is known to all that L1 cache provides the least latency, it is still an interesting question what is the worst situation that still exposes an attack window.

The second factor is type of exception. Different types of exceptions may yield different exception handling traces, and corresponding latency may vary. Different exceptions also correspond to different threat models and attacks. What's more, one single instruction could have multiple exceptions and such exceptions may also lead to possible attack window for different types of attacks.

The last part overlaps with those that affect exception handling latency. In specific, availability of different levels of TLB and availability of paging structure in different levels of cache or memory all lead to different attack window width. Such factors influence data fetching in that data could only be fetched after a virtual address finishes its translation into its physical address. Meanwhile, the access controls are most set by bits in the PTE entry and thus exception handling also needs to wait until the translation finishes. As a result, there is a bi-directional impact on the attack window.

\subsection{Speculative Execution Depth}
\label{subsec:depth}

\begin{lstlisting}
movapd \%xmm0, \%xmm1
addpd \%xmm1, \%xmm0
mulpd \%xmm1, \%xmm0
movapd \%xmm0, \%xmm1
addpd \%xmm1, \%xmm0
mulpd \%xmm1, \%xmm0
...
[cpuid]
// %rsi stores the illegal address
movzx (\%rsi), \%rax
mov \$1, \%rbx
mov \$1, \%rbx
[cpuid]
mov \$1, \%rbx
...
\end{lstlisting}

We measure the capability of speculative execution, i.e. how many micro operations could be executed speculatively following a faulty instruction, with the help of performance of performance counters. The two events we monitor are UOPS\_EXECUTED.THREAD and UOPS\_ISSUED.ANY. The performance counters monitoring is supported with the help of PAPI. The depth of speculative execution is decided by how soon the exception of the faulty instruction is captured. According to our observation in \ref{subsec:model_verification} and Intel manuals, exception handling mechanism is applied as soon as the processor captures the exception. The issuing of instructions stop right away and the frontend is re-directed to fetch the exception handler code. Thus, issued \uops reflects the latency of exception capturing. But we should notice that the size of ROB sets a limitation to the issuing of instructions. If the ROB is full, issuing has to wait until the first instruction in ROB retires and gets cleared from ROB. To avoid this limitation as much as possible, we make sure the faulty instruction is the first one in ROB. But since it will never retire, the fetching of speculated instructions will be at most {SIZE\_OF\_ROB-1}.

Since it is impossible to directly monitor exactly the speculatively executed instructions, the methodology is to perform a controlled differential analysis. The monitoring starts before the faulty instruction and ends at the beginning of a user-specified segfault handler.

The code to be monitored is made up of three components: preceding instructions, a faulty instruction and speculative instructions. In \ref{subsec:retirement} we will show that the influence of preceding instructions could be ignored. But in this experiment we still put a sequence of inter-dependent float-point computation instructions before the faulty instruction. Meanwhile, a CPUID instruction could be optionally inserted after them to ensure a clean ROB at the fetching of the faulty instruction. An assumption is that the CPUID instruction could work correctly as described in Intel's manual to ensure that all execution results before it are posted to any registers, cache or memory, before fetching the next instruction.

For the faulty instruction, we choose a simple instruction of "movzx (\%rsi), \%rax", where an illegal kernel virtual address is stored in register \%rsi.

The speculative instructions are all simple "mov \$1, \%rbx". They are independent on any instructions including the faulty instruction. Upon their issuing, their execution could start right away and the execution time remains constant. Among the speculative instructions, CPUID could be inserted to limit the number of speculative instructions and verify the PC readings change accordingly.

The experiment results suggest that with different desired speculative execution depth, both PC event readings change accordingly and are very close to each other. Thus, it is feasible to perform differential analysis for the purpose of further experiments using this method. However, there is a limitation to this method. The PC events are unable to reveal the real number of executed micro-ops. It includes both executed micro-ops and squashed micro-ops. Details are explained in \ref{subsec:tool_verify}.



\subsection{Data Available Latency Measurement}

One last missing piece regarding the execution model is a proper method to measure the latency for data to be available for following instructions dependent on it to use.

\subsubsection{Covert-Channel-Based Differential Analysis}

\begin{lstlisting}
// %rdi stores the address to the covert channel buffer
sub \$M, \%rdi
// (%rsi) stores the illegal address
movq (\%rsi), \%rsi
movzx (\%rsi), \%rax

// there are M add instructions
add \$1, \%rdi
add \$1, \%rdi
...
add \$1, \%rdi
mov (\%rdi), \%rdx
\end{lstlisting}

The flush-reload covert channel provides us with a reliable way to know exactly whether an instruction is executed or not. We need to make an assumption that when CPU captures an exception, the following instructions will be squashed immediately. And based on the experiment results in \ref{subsubsec:issue_execute}, if an instruction has not finished its execution by the time it is squashed, it won't be executed any more. Thus, we are able to infer when the exception is captured by counting how many instructions are successfully executed. This serves as the basis of our experiment design to measure the latency for the data to become available for following instructions dependent on it.

The key insight in this method is that instead of measuring the time for the illegal data to come, we measure the time for some legal data to become available. And the legal data is exactly the illegal virtual address that we trigger an exception by accessing it. Thus, we are able to measure the total time from executing a first instruction to read the virtual address into a register to CPU capturing the exception caused by the second instruction trying to access the illegal virtual address.

The address of the memory buffer that stores the illegal virtual address is loaded into a register, say \%rsi. The above strategy could be realized by forming an instruction sequence of a "movq (\%rsi), \%rsi" and a "movzx (\%rsi), \%rax".

Following these, a series of speculative instructions of "add \$1, \%rdi" are attached. A covert channel memory buffer is required and we store its address right in the register \%rdi. Thus, after them we should have a "mov (\%rdi), \%rdx" to access the buffer. We can change the number of such ADD instructions to find the maximum that still allows the final MOV instruction to be executed. One thing to notice is that in order to maintain correctness after we change the number of the ADD instructions, we should correspondingly change the address originally stored in \%rdi. For example, if we wish to insert 7 such ADD instructions, the original data in \%rdi should be "covert\_buffer\_address - 7".

If we change the conditions such as caching and TLB availability, we could differentially know the relative data abailable latency, considering that we could control the exception capture latency.

\subsubsection{CPU-Idle-Cycle-Based Differential Analysis}

\begin{lstlisting}
cpuid
// in total 65 movq instructions
// the last movq is illegal
movq (\%rax), \%rax
movq (\%rax), \%rax
movq (\%rax), \%rax
...
movq (\%rax), \%rax
cpuid
\end{lstlisting}

Another method we design to measure the latency of data arrival for speculative execution is to make use of a performance counter events called UOPS\_EXECUTED.STALL\_CYCLES. It measures the number of cycles where there are no micro-ops being executed. By making the following issued instruction wait due to data dependency, we are able to tell how many cycles it takes for the data to arrive. And we amplify the signal by creating a chained list and accessing them using a series of instructions "movq (\%rax), \%rax". This ensures that when one of these MOVQs is fetching data, none of latter instructions could be executed at the same time. We also add before and after this code snippet a CPUID instruction to eliminate the influence of other instructions. Note that in order to fit into the design that the end of monitoring is set in the exception handler, the data stored in the second last address is set to be an illegal virtual address. Thus, the last MOVQ is going to trigger an exception.

Our experiment results suggest that when changing the caching and TLB conditions, we could differentially measure the difference in the idle cycles for fetching data. One assumption here is that other instructions within the monitoring period always yield the same or similar number of idle cycles. Since all other code remains the same, this assumption is reasonable to some extent, despite a little fluctuation. To make the experiment more dependable, we relieve the reliability on this assumption by extending the MOVQ instruction sequence so that the true signal of idle cycles caused by waiting for data is strong enough to ignore the influence of other instructions.

\subsection{Attack Window Measurement}

\begin{lstlisting}
movq (\%\%rcx), \%\%rax
[add \$1, \%\%rax]
[add \$1, \%\%rax]
[...]
[add \$1, \%\%rax]
movq (\%\%rbx, \%\%rax, 1), \%\%rbx
\end{lstlisting}

Based on the generic speculative side-channel vulnerability analysis, we design another method that could specifically measure the vulnerability window of meltdown attack in number of instructions. It could also be converted into the finer grained number of micro-ops with the help of IACA.

Consider the following code snippet of a typical meltdown attack:
"movzx (\%\%rcx), \%\%rax", 
"shl \$12, \%\%rax", 
"movq (\%\%rbx, \%\%rax, 1), \%\%rbx".
In register \%RCX stores an illegal kernel mode virtual address and in register \%RBX stores the virtual address of the beginning of a flush-reaload covert-channel memory buffer. To measure the attack window, we slightly modify it to eliminate unnecessary side effect of out-of-order execution. We replace the first instruction with "movq (\%\%rcx), \%\%rax". Suppose originally the one-byte data stored at the address is \$23, we substitute it with an eight-byte (64-bit) data of (\$23 << 12). And we remove the second instruction, keeping only the third instruction.

In order to measure how late the secret data could still be effectively used as the offset to the covert-channel buffer, we insert between the two instructions a series of "add \$1, \%\%rax". The ADD instructions are all inter-dependent and their execution involves only one single computation unit and nothing else. They serve as a good candidate for measurement because they do not introduce side effects.

After returning from the exception handler, we do a reload on the expected memory buffer slice to check whether it is accessed. We also inspect the buffer slice corresponding to data 0 to observe the zero-out effect. By changing the length of ADD instructions, we observe when the buffer starts to be unable to be accessed speculatively. Then the attack window is exactly the number of such ADD instructions. When we change the caching and TLB conditions, the attack will also change accordingly.

\subsection{Fuzzer Model}

\subsubsection{Faulty Instruction Model}
\label{subsubsec:instruction_model}

Each entry in the exception and protection list in \ref{subsec:exception_protection} could be modeled into an instruction template, as in Table \ref{tab:instruction_model}. As long as there are no conflicts in the models of two rules, they could be combined into one single instruction.

\begin{table*}[t]
\centering \footnotesize{
\begin{tabular}[t]{c|c|c|c|c|c|c|c|c}
\Xhline{1pt}
Index & Instruction & Operands & CPU mode & Page table & 
Control Registers & Features & Other & Trigger stage  \\
\Xhline{1pt}
1 & & M(r)/M(w) & & P = 0 & & & & Execution \\
2 & & M(r)/M(w) & & Reserved = 1 & & & & Execution \\
3 & & M(r)/M(w) & Supervisor & U/S = 0 & CR4.SMAP = 0 & PK forbid & & Execution \\
3 & & M(r)/M(w) & Supervisor & U/S = 0 & CR4.SMAP = 1 & & EFLAGS.AC = 0 & Execution \\
4 & & M(r)/M(w) & Supervisor & U/S = 0 & CR4.SMAP = 1 & & Implicit access & Execution \\
5 & & M(r)/M(w) & Supervisor & U/S = 0 & CR4.SMAP = 1 & PK forbid & EFLAGS.AC = 1 & Execution \\
\multirow{2}{*}{6} & & \multirow{2}{*}{M(w)} & \multirow{2}{*}{Supervisor} & U/S = 0 & & & & \multirow{2}{*}{Execution} \\
& & & & W/R = 0 & & & & \\

\multirow{2}{*}{7} & & & \multirow{2}{*}{Supervisor} & U/S = 1 & & & PAE OR IA-32e w/ & \multirow{2}{*}{Fetching} \\
& & & & XD = 1 & & & IA32\_EFER.NXE = 1 & \\

8 & & & Supervisor & U/S = 0 & CR4.SMEP = 1 & & & Fetching \\
\multirow{2}{*}{9} & & & \multirow{2}{*}{Supervisor} & U/S = 0 & \multirow{2}{*}{CR4.SMEP = 0} & & PAE OR IA-32e w/ & \multirow{2}{*}{Fetching} \\
& & & & XD = 1 & & & IA32\_EFER.NXE = 1 & \\

10 & & M(r) & User & & & PK forbid & & Execution \\
11 & & M(r) & User & U/S = 1 & & & & Execution \\
12 & & M(w) & User & R/W = 0 & & & & Execution \\
13 & & M(w) & User & & & PK forbid & & Execution \\
14 & & M(w) & User & U/S = 1 & & & & Execution \\
\multirow{2}{*}{15} & & & \multirow{2}{*}{User} & \multirow{2}{*}{XD = 1} & & & PAE OR IA-32e w/ & \multirow{2}{*}{Fetching} \\
& & & & & & & IA32\_EFER.NXE = 1 & \\

16 & & & User & U/S = 1 & & & & Fetching \\
17 & & M(r)/M(w) & SGX & & & & Illegal virtual address & Execution \\
\multirow{2}{*}{18} & & \multirow{2}{*}{M(r)/M(w)} & \multirow{2}{*}{SGX} & & & & Target EPC page not  & \multirow{2}{*}{Execution} \\
& & & & & & & within current enclave & \\

19 & & M(r) & SGX & & & & EPCM denies read & execution \\
20 & & M(w) & SGX & & & & EPCM denies write & execution \\
21 & & & SGX & & & & EPCM denies execute & fetching \\
\multirow{2}{*}{22} & & \multirow{2}{*}{M(r)/M(w)} & \multirow{2}{*}{SGX} & & & & PT\_SECS/PT\_TCS/ & \multirow{2}{*}{Execution} \\
& & & & & & & PT\_VA/PT\_TRIM page & \\

\multirow{2}{*}{23} & & \multirow{2}{*}{M(r)/M(w)} & \multirow{2}{*}{SGX} & & & & BLOCKED/PENDING/ & \multirow{2}{*}{Execution} \\
& & & & & & & MODIFIED page state & \\

\multirow{2}{*}{24} & & & \multirow{2}{*}{SGX} & & & & Fetch code from virtual & \multirow{2}{*}{Fetching} \\
& & & & & & & address outside enclave & \\

\multirow{2}{*}{25} & & & \multirow{2}{*}{SGX} & & & & Fetch code splitting & \multirow{2}{*}{Fetching} \\
& & & & & & & across ELRANGE bound & \\

26 & & & & & & & Instruction length limit & Fetching \\
\multirow{2}{*}{27} & \multirow{2}{*}{MOV} & R(r) & & & CR0.PG = 1 & & & \multirow{2}{*}{Execution} \\
& & CR(w) & & & CR0.PE = 0 & & & \\

\multirow{2}{*}{28} & \multirow{2}{*}{MOV} & R(r) & & & CR0.NW = 1 & & & \multirow{2}{*}{Execution} \\
& & CR(w) & & & CR0.CD = 0 & & & \\

\multirow{2}{*}{29} & \multirow{2}{*}{MOV} & R(r) & & & CR4.Reserve & & & \multirow{2}{*}{Execution} \\
& & CR(w) & & &  = 1 & & & \\

\multirow{10}{*}{30} & LGDT/LLDT/ & & \multirow{10}{*}{Non-S} & & & & & \multirow{10}{*}{Execution} \\
& LTR/LIDT/ & & & & & & & \\
& LMSW/CLTS/ & & & & & & & \\
& INVD/HLT/ & & & & & & & \\
& WBINVD/ & & & & & & & \\
& INVLPG/ & & & & & & & \\
& RDMSR/ & & & & & & & \\
& WRMSR/ & & & & & & & \\
& RDPMC/ & & & & & & & \\
& RDTSC/ & & & & & & & \\

\multirow{4}{*}{31} & \multirow{4}{*}{MOV} & CR(r)/ & \multirow{4}{*}{Non-S} & & & & & \multirow{4}{*}{Execution} \\
& & CR(w)/ & & & & & & \\
& & DBG(r)/ & & & & & & \\
& & DBG(w) & & & & & & \\

32 & WRMSR & & & & & & MSR.reserve = 1 & Execution \\
\multirow{2}{*}{33} & \multirow{2}{*}{MOV} & \multirow{2}{*}{CR(w)} & & & CR4.PAE = 1/ & & PDPT.reserve = 1 & \multirow{2}{*}{Execution} \\
& & & & & CR4.PSE = 1 & & CR0, CR3, CR4 only & \\

34 & (V)LDMXCSR & M(r) & & & & & MXCSR.reserve = 1 & Execution \\
35 & SSE(1/2/3) & M(r) & & & & & Addr not 128-bit aligned & Execute \\
\Xhline{1pt}
\end{tabular}} \\[4pt]

\begin{minipage}{1.98\columnwidth}
\centering
\caption{Instruction model. Not yet including DE, DB, UB, NM, SS and non-exceptional protections.}

\label{tab:instruction_model}
\end{minipage} \\[-10pt]
\end{table*} 


==> tex/backup-sgx.tex <==

\subsubsection{Non-exceptional Protections}

\yx{This section may be too verbose.}

Some hardware protection schemes do not raise an exception when violation is found by the processor. Instead, it is handled silently by the processor itself to hide the secret. This is most common in the security protocol of hardware extensions such as SGX.

The TLB miss handling process of SGX is a typical example of such non-exceptional protections. It is an extension of the common PMH (Page Miss Handler). When a process out of enclave tries to access an enclave address, the virtual address needs to be translated into physical address first. As in common paging translation, TLB is referred to for the corresponding entry. In the absense of the requested TLB entry, the common PMH performs page structure walk and create an entry in the TLB. If the TLB is already available in the first place, this step is not needed. Any security checks can begin only after the TLB entry is present. (Checks on higher level page structure entries are not considered here.)

Page table access privilege checks are first conducted. Afterwards, SGX performs enclave-related security checks to determine whether the access is allowed. If violations are discovered, the TLB entry will be silently replaced by one pointing to a physical page full of 1. That way, any accesses to it can only get a data of -1 without triggering exceptions.

However, the hardware implementation of such schemes is not clear and in fact contains bugs, leading to exploitation such as foreshadow attack. We conducted several experiments to study how exactly it is implemented and explain the attack in a systematic way with the help of our model. We constructed an access to an enclave address from outside the enclave, similar to the settings of foreshadow. The access suppressing method is Intel TSX. The data loaded by the illegal access is then used as an index to a covert channel buffer by the following instruction. For all our experiments, we ensure that the enclave data is in L1. 

\begin{lstlisting}[caption={Foreshadow attack nature experiment.},label={lst:foreshadow}]
// %RBX: address of uncached covert channel buffer
// %RCX: enclave address whose data is 0x42
// To capture data of -1, we add a 5 to it.
// Covert channel expects either 0x47, 0x5 or 0x4,
// corresponding to correct value, 0 or -1.
[clear P flag]
[xbegin]
movq (%rcx), %rcx
add $5, %rcx
shl $12, %rcx
movq (%rbx, %rcx, 1), %rcx
[xend]
\end{lstlisting}

We performed three sets of experiments, each repeated for several hundred times to ensure reliability. A common form of the experiment code is shown in \lstref{lst:foreshadow}. In the first set of experiments, we take the traditional foreshadow attack settings. The illegal access to enclave memory is wrapped in a TSX transaction and the P flag of the PTE of the accessed page is cleared. Flush-reload covert channel after executing the illegal access finds that the data given by the access to enclave are mostly (over 2/3) the expected value and the rest zero. This is as expected according to the original attack paper. 

In the second set of experiments, the illegal access is still wrapped by TSX transaction but the P flag is not cleared. With P flag set, the page fault exception will not be triggered. And we found that in all of the tests only zero value is captured by the covert channel. 

In the third set of experiments, the TSX transaction is removed and the P flag is not cleared. In this case, in all of the tests, the covert channel buffer entries corresponding to both 0 and -1 are touched. 

From experiment 2 and 3, we are able to see that TSX transaction aborts before the TLB entry is replaced to point to the dummy page full of 1. And interestingly, the illegal access first returns a zero value for the speculative execution of following instructions but later corrects it after substituting the TLB entry. What's more, if we compare them with experiment 1, it is even more interesting in that with P flag uncleared, no accesses could fetch the correct data even when it is in L1 cache. According to our two-phase exception handling model, zero data is provided if data fetching latency is greater than \phaseone latency. Otherwise, correct data will be fetched first. With that in mind, we could see that when accessing enclave memory from outside, the race between \phaseone and data fetching is always winned by \phaseone when there are no other interference. But after involving the terminal fault caused by clearing the P flag, there is a chance for the data fetching to win. However, since the data is ensured to be kept in L1 cache, the only explanation is that the terminal fault caused by clearing P flag has two functions here. One is that it terminates further SGX check and the other is that it slows down \phaseone.

One possibility for this to happen is that in the hardware implementation, the SGX check is performed after paging checks finish rather than done in parallel at the same time. And both checks, without considering the extra time for processor to deal with them, are really fast. When no faults or non-terminal faults are captured, the SGX check is performed and the total \phaseone latency is still less than L1 data fetching latency. On the other hand, when there is a terminal fault caused by an unset P flag, the processor needs extra time to deal with it. Meanwhile, the fast SGX check is not performed to override it. This leads to the result that the \phaseone latency reflects only the non-present fault. This also explains why other causes of page faults cannot work in L1TF attack.

Extended page table (EPT) for VMX works in a similar way as SGX. Designing hardware extensions by directly attaching them to existing architecture may be straightforward but not secure, especially for the security-sensitive SGX. To enforce SGX protection, a better design is that SGX check begins right after TLB entry is available in parallel with paging checks.

==> tex/backup-tool.tex <==
\subsection{Tool Verification}
\label{subsec:tool_verify}
\yx{discard this subsection}

\textbf{Performance counter semantics verification.}
We rely on performance counters for some experiments. Accuracy of performance counters is not critical in our experiments, but there are still issues that we need clarify before we experiment with them. One issue is that different architectures have different monitoring events. The events we are interested in may not be available on tested platforms or have different names. We need to check correspondingly before using the events and find substitutes if they are not available. The other issue is that the true semantics of specific events may be uncertain. For example, on one of our test machines, the event counting the number of executed micro-ops in fact include both executed and squashed micro-ops which are not executed speculatively after exception is captured by the CPU. This needs to be verified with ground truth we get from covert channel.

\subsubsection{UOPS\_EXECUTED PC Analysis}

\begin{lstlisting}
cpuid
// %rsi stores the illegal address
movzx (\%rsi), \%rax
movq (\%rax), \%rax
movq (\%rax), \%rax
movq (\%rax), \%rax
...
\end{lstlisting}

In order to understand the true meaning of the performance counter events, we perform some more experiments in additional to the covert channel experiments. We remove the covert channel instructions and replace them with a long sequence of interdependent instructions. And the actual number of issued and executed instructions are counted using the performance counter events in the view of micro-ops.

The whole instruction sequence is as below. An CPUID instruction is put before the faulty instruction to eliminate unnecessary influence, although in fact preceding instructions won't affect CPU's capture of the exception, which is explained in \ref{subsec:retirement}.

The faulty instruction is a "movzx (\%rsi), \%rax". The speculative instructions are all "movq (\%rax), \%rax" to create a inter-dependent instruction sequence. The real data stored at the illegal address specified by \%rsi points to the beginning of a linked list. Obviously, since the linked list is finite, the last instructions will try to access an invalid virtual address. But the problem could be ignored as long as the list is long enough. If the assumption that any issued instruction will be speculatively executed unconditionally, it does not matter if the speculative instruction itself is faulty or not. And we could immediately notice it from the reading of the performance counters if this is not true.

We control the latency from the beginning of execution of the faulty instruction to CPU's capturing of the exception to be constant. This ensures that the issue of following instructions remain the same until the ROB is full. An assumption here is that the fetch, decode and issue of instructions are not affected by backend execution except for the limit of ROB size.

At the same time, we change whether the data at the illegal address is in cache or in memory to change the latency of speculative execution since all instructions have to wait until dependency is resolved to be executed.

From the performance counters, we notice that both the number of issued micro-ops and the number of executed micro-ops always remain constant when we change the caching status. The first number is as expected. But the second number shows that in fact squashed micro-ops are also counted as executed although they are not actually executed, if we compare the results with the ground truth we got from \ref{subsubsec:issue_execute}.


==> tex/backup-understanding.tex <==
\section{Understanding \vulname Vulnerabilities}
\label{sec:understanding}

%To explore the \vulname vulnerabilities of a variety of Speculation Primitives on multiple processor micro-architectures, \sysname conducts a set of tests for each of the combination of the Speculation Primitives and processor micro-architectures. The tests are designed atop the basic instruction execution model described in \secref{sec:method:model}, but are intended to deepen our understanding of the \vulname vulnerabilities to go beyond the vendors' manual and patent disclosure. 

%Exception handling process is the key to transient execution attacks. However, the detailed implementation is not well documented and may vary from platform to platform. Thus, it is crucial to verify several facts and understand how we could manipulate the latency of exception handling operations by the processor.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{fig/tests.png}
\caption{The overall organization of tests.}
\label{fig:tests}
\end{figure}

\vulname vulnerabilities are caused by speculative execution. However, being able to speculatively execute instructions itself does not qualify a vulnerability. The root cause of  \vulname vulnerabilities is that some secret data not supposed to be accessed could be accessed by speculatively executed instructions. Moreover, once the secret data is accessible to the speculative instructions, what can be done with it (\eg, leaking the secret using covert channels) is determined by the attack window---the time period (in CPU cycles) from the first speculative instruction being executed to the termination of all speculative instructions. Therefore, to understand \vulname vulnerabilities, their \textit{exploitability} and \textit{attack window} must be quantitatively measured. %we envision one must understand three categories of questions: First, what is the root cause of a \vulname vulnerability, how to measure it, and how to control it from the software? Second, what determines the window of speculative execution, how to measure the speculation window, and how to control (\eg, enlarge) it? Third, what is the side effects of one exploitation of the \vulname vulnerability on future ones?

\yx{TODO: make sure the term "attack window" is accurate}
In this paper, we aim to use the two-phase model described in \figref{fig:two-phase} to explain and measure the \textit{exploitability} and \textit{attack windows} of the \vulname vulnerabilities. To establish the relationship, we designed four tests under the \sysname framework (shown in \figref{fig:tests}) to determine what effects \phaseone and \phasetwo of the Speculation Primitive have on the current execution unit and other execution units, respectively.

%To answer these questions, we designed 10 tests in the \sysname framework. The relationship between questions and tests are illustrated in \figref{fig:tests}. To understand what determines the \vulname vulnerability, we run tests to understand what effects \phaseone and \phasetwo of the Speculation Primitive have on the current execution unit and other execution units, respectively. \textit{The empirical results suggest that relative latency of \phaseone, compared to the latency of secret data access, determines whether or not the underlying Speculation Primitive leads to an exploitable vulnerability. } 

To measure the exploitability of the \vulname vulnerabilities, we perform a test to measure the relative \phaseone latency to data fetching and another test to quantify it.  To measure the attack windows of the \vulname vulnerabilities, we perform a test to measure the \phasetwo latency.
%To understand what determines the attack windows, we perform tests to explore the effect of \phaseone and \phasetwo on the entire execution engine. The conclusion is that the size of the attack window is determined by \phasetwo, which can be measured and altered. 

Finally, to study the side effect of speculative instructions, we test how caches are affected by the speculative instruction. This helps us understand how one round of attacks may help the subsequent ones. 


%The first experiment is to prove the existence of \phaseone. Contrary to the well-known existence of \phasetwo at retirement for exception handling, \phaseone is never suggested in any previous study, yet critical to \atkname, and is not documented in processor vendor manuals. We are going to demonstrate its existence by leveraging its major effect of influencing data fetching. In the second experiment, we extend the study of the effect of \phaseone to clarify the uncertainty about its other effects. Then our third experiment turns to \phasetwo and prove the hypothesis on the effect of it.

%Afterwards, we carry out the measurement on \phaseone which determines whether a potential variant is exploitable or not. And we also present a method to study the important question of whether \phaseone could be changed to facilitate the attack. It is known that \phasetwo could be changed by controlling the retirement, but we hereby quantitatively measure the exact relationship between retirement latency and attack window which is decided by \phasetwo latency.

%Notice that different variant corresponding to different exceptions may have different characteristics regarding these experiments. Thus, we leverage \sysname to enable tests on different kinds of variants. 

The \sysname framework allows running each of the tests described in this section to examine different types of Speculation Primitives corresponding to different variants. For the clarification and simplicity of discussion, in this section, we describe these tests using a Speculation Primitive similar to the one used in the Meltdown-US attack \cite{Lipp2018meltdown}. 
\yx{added something here}
Note that the front end components of the execution engine (such as IDQ) do influence our tests, but we only need to control ROB, which is directly connected to the execution component of the engine. Before executing the instruction sequence of each test, we use a CPUID to make sure the ROB is empty. We will point out other controls should they be needed for specific tests.

% as an example and we will point out when certain variants yield different results. The results of the experiments are presented in \secref{sec:evaluation}.

% Following the speculative instruction handling mechanism is another important question of the relationship between exception and retirement. Whether the processor deals with the exception immediately after it captures it or it waits until the retirement of the speculation primitive influences the vulnerability directly. By experiments, we find that the exception handling has two phases, as described in \secref{subsec:handling}. The attack window could be expanded by delaying the retirement with slow windowing gadget but the exploitation of the vulnerabilities rely on availability of the true secret data, \ie the first phase of exception handling. \yx{this paragraph is moved from somewhere else to here}




\subsection{\phaseone on Current Execution Unit}
\label{subsec:e1_existence}

\bheading{Test goals.}
This test is designed to determine how \phaseone affects the execution unit being used by the Speculation Primitive. 

\begin{lstlisting}[float=htbp,caption={The effects of \phaseone on the current execution unit.},label={lst:phaseonecurrent}]
 // %RBX: address of uncached covert channel buffer
 // (%RBX-0x40): address of uncached data
 // *(%RBX-0x40) = %RBX
 // %RCX: illegal address whose data is 0x42000
 // ---------------------------------------------
 // Windowing Gadget 
     sub %rbx, %rcx
     sub $0x40, %rbx
     movq (%rbx), %rbx
 // ---------------------------------------------
 // Speculation Primitive
     movq (%rbx, %rcx, 1), %rcx
 // ---------------------------------------------
 // Disclosure Gadget
     movq (%rbx, %rcx, 1), %rbx
\end{lstlisting}

\bheading{Instruction sequences.}
As shown in \lstref{lst:phaseonecurrent}, the instruction sequence consists of a Windowing gadget, a Speculation Primitive, and a Disclosure Primitive. The Speculation Primitive includes two SUB instructions to prepare the desired register values. Because all the subsequent instructions have dependency on the data read by the Windowing Gadget, they start execution as soon as the data fetched by the Windowing Gadget becomes available, but not before that. %As the instruction issuing is not stalled by the Windowing Gadget, which will continue until the ROB is full, the Windowing Gadget makes sure the execution of following instructions is not delayed due to instruction issuing. 

%the Speculation Primitive is a simple MOV instruction to access a secret value from an illegal address (\eg, a kernel-space address) to a register. Following it is the Disclosure Gadget which consists of one single instruction to access a data array according to the secret value. The Windowing Gadget is used to eliminate the side effect of instruction issuing. 
%Because the Disclosure Gadget is used to reflect the execution time of speculatively executed instructions, it is desired that the instructions in the Disclosure Gadget are not stalled because they are yet to be issued into the ROB. To address this problem, the Windowing Gadget contains a memory read to an uncached memory address. 

%\yz{why use two sub instructions in the Windowing Gadget? Can you explain in details about the code?} \yx{(Refer to the comments in the listing) Before executing them, the register RBX stores the address of the covert channel buffer and register RCX stores the address that is not allowed to access. The first SUB intends to turn the speculation primitive to be dependent on the windowing gadget. After executing it, (RBX+RCX) to be accessed by the speculation primitive will be illegal address again. The second SUB instruction makes the address in RBX to point to a different cacheline (flushed to memory) outside the covert channel buffer. But the data stored at that cacheline is in fact the address of the covert channel buffer. Thus, executing the windowing gadget will push the address of the covert channel buffer back to RBX.}



% The experiment design is similar to \ref{subsubsec:issue_execute}. Following a slow memory load is a speculation primitive depending on the slow data. And in the end is also a load of covert channel buffer. However, it is different in that the inserted ADD/SUB instructions and the final MOV are all dependent on the illegal data. As a result, they only begin execution after the data becomes available by the speculation primitive. We measure the attack window by counting the maximal number of inserted ADD/SUB instructions that still allow the covert channel load instruction to execute.



\bheading{Experiments and expected observations.}
The tests were repeated four times, with the secret data placed in the L1 cache, L2 cache, the LLC, and the memory, respectively. The TLB entry of the secret address is always flushed to ensure a fixed \phaseone latency. In these experiments, we would hope to see whether the change of the data fetching latency affects the covert-channel signal received by the Disclosure Primitive. If so, whether \phaseone happens before or after the data fetching is completed affects the return values of current execution unit. 

% is later than the data latency, we expect to read the correct secret data from the covert channel; otherwise, we expect to see some changes in the secret data.


\ignore{
\subsection{Effect of \phasetwo on current execution unit}

\bheading{Test goals.}
In order to conclude that \phaseone is the sole factor that could stop the execution unit that triggers the exception, we need to prove that the data fetched has nothing to do with \phasetwo.

\bheading{Experiments and expected observations.}
\yx{here should be a simple experiment using code from \secref{subsec:e2_change} but observe whether the captured value change from the correct value to zero. The result is included in \secref{subsec:e2_change_eval}.}
}


\subsection{\phaseone on Other Execution Units}
\label{subsec:e1_effect}


\bheading{Test goals.}
This test aims to determine whether %\phaseone affects the execution unit that causes the exception. 
% In this test, we hope to determine whether \phaseone also influences other components of the execution engine, \ie whether the processor also squashes speculative instructions in ROB and/or the switching to exception handling code of the front end. 
\phaseone affects other execution units. If that is the case, attacks may be enhanced by combining two or more Speculation Primitives.

\bheading{Instruction sequences.}
Different from other tests, two Speculation Primitives are included in this test to determine whether \phaseone of the first Speculation Primitive also influences the execution of the execution unit used by the second Speculation Primitive. We consider two cases, depending on whether the two Speculation Primitives access the same memory address.

First, the two Speculation Primitives access the same memory address. The instruction sequence is designed as shown in \lstref{lst:sameaddress}. A sequence of inter-dependent ADD/SUB instructions are inserted between the two Speculation Primitives to control the delay of the execution of the second Speculation Primitive. Since these inserted ADD/SUB instructions and the first Speculation Primitive all depend on the Windowing Gadget, they all start at the same time. But the second Speculation Primitive has to wait until all the ADD/SUB instructions finish. The Disclosure Gadget is used to measure the speculation window of the second Speculation Primitive. %To make sure \phaseone and \phasetwo of the first speculation primitive are distant enough for such potential zero phenomenon, we place a slow memory load instruction in the windowing gadget before the first speculation primitive to delay its retirement.

\begin{figure}[tb]
\centering
\includegraphics[width=\columnwidth]{fig/phaseone_on_other.png}
\caption{Illustration of \phaseone effects on other execution units.}
\label{fig:phaseone_on_other}
\end{figure}

Second, the two Speculation Primitives access different memory addresses. The instruction sequence used is the same as the first case, except for the memory addresses accessed by the two Speculation Primitives. 



%Then we observe the execution of the second speculation primitive by using its data as the index to the covert channel buffer. In order to control the delay for the second speculation primitive to begin execution, we add between the two speculation primitives a sequence of inter-dependent ADD/SUB instructions. Common start of the inserted instructions and the first speculation primitive is enforced by the windowing gadget. The second speculation primitive has to wait until all the ADD/SUB instructions finish execution to get started. 

\begin{lstlisting}[float=htbp,caption={The effects of P1 on the other execution units},label={lst:sameaddress}]
 // %RBX: address of uncached covert channel buffer
 // (%RBX-0x40): address of uncached data
 // *(%RBX-0x40) = %RBX
 // (%RBX+0x3000): address of uncached data
 // %RCX: illegal address #1 whose data
 // %RAX: illegal address #2 whose data is 0x42000
 // ---------------------------------------------
 // Windowing Gadget
     sub %rbx, %rax
     sub %rbx, %rcx
     sub $0x40, %rbx
     movq (%rbx), %rbx
 // ---------------------------------------------
 // Speculation Primitive #1
     movq (%rcx, %rbx, 1), %rcx
 // ---------------------------------------------
 // special inserted instructions for the experiment
     add %rbx, %rax
     [add $1, %rax]
     [sub $1, %rax]
     ...
 // ---------------------------------------------
 // Speculation Primitive #2
     movq (%rax), %rax
 // ---------------------------------------------
 // Disclosure Gadget
     movq (%rbx, %rax, 1), %rbx
\end{lstlisting}

\bheading{Experiments and expected observations.} In both tests, the relevant data are stored in the L1 cache. As shown \figref{fig:phaseone_on_other}, the events with black labels describe the first Speculation Primitive, and the ones with red labels describe the second. By delaying the execution of the second Speculation Primitive, \phaseone of the first Speculation Primitive can happen before the second Speculation Primitive fetches the secret data. Therefore, in the experiment, we will gradually insert more instructions between the two Speculation Primitive and observe whether at certain point the Disclosure Primitive catches a zero signal. If so, it must be caused by \phaseone of the first Speculation Primitive. 

%If \phaseone of the first Speculation Primitive could also stop the execution of the second, by delaying the execution of the second speculation primitive to the circumstance shown in \figref{fig:phaseone_on_other} we expect a data of 0 to occur. 

%We test with the data accessed by the first speculation primitive in either L1D or in L2, while we force the data of the second instruction to be in L1D. Similarly to the first case, we still observe whether the zero phenomenon could appear when we gradually change the latency of the second speculation primitive. 

% \begin{lstlisting}[caption={Influence of \phaseone on another access to a different address},label={lst:diffaddress}]
% // %RBX: address of uncached covert channel buffer
% // (%RBX-0x40): address of uncached data
% // *(%RBX-0x40) = %RBX
% // %RCX: illegal address whose data is 0x42000
% // (%RCX+0x140): another illegal address whose data is 0x42000
% mov %rcx, %r8
% add $0x140, %r8
% sub %rbx, %r8
% sub %rbx, %rcx
% sub $0x40, %rbx
% movq (%rbx), %rbx
% movq (%rcx, %rbx, 1), %rcx
% add %rbx, %r8
% [add $1, %r8]
% [sub $1, %r8]
% ...
% movq (%r8), %r8
% movq (%rbx, %r8, 1), %rbx
% \end{lstlisting}






\subsection{\phasetwo on Execution Engine}
\label{subsec:e2_effect}

% \yx{the two experiments are conducted together but observe different things}

\bheading{Test goals.}
This test is designed to determine the effects of \phasetwo on the entire execution engine. 

%Compared to \phaseone, the fact that \phasetwo is involved in exception handling is well known. For a given exception on a given processor, \phasetwo controls the squashing of the speculative instructions in case of an exception. The exact relationship between \phasetwo latency and squashing latency is looked into in \secref{subsec:e2_change}. Here we only prove whether issued but unexecuted instructions are allowed to finish their execution, \ie whether they are squashed or not. The processor may or may not always execute all issued instructions. If it does so, malicious code will always be executed as long as it is issued and the attack will become easier. But this situation is generally thought untrue and we could verify it with experiments.



% \yx{this paragraph is not useful}
%\ignore{With previous knowledge on meltdown attacks, an observation is that after CPU notices that an instruction violates the access control policy, the data put into register will be zero-ed out. However, this scheme is in fact not well studied. There are still uncertain questions. Is the zero value always provided by the CPU as data regardless of whether the data is already read into the target register at the time when CPU captures the exception? Will all issued instructions always be executed using the zero value if they have data dependency on the speculation primitive? The first question is hard to verify since the internal states of the CPU are hidden from us, but luckily for this project it is not critical. The zero value will possibly be used only after CPU captures an exception. For the attacker, if the data is not yet available at that moment, it does not matter whether zero is applied. So still the only thing we care about is whether the data is already available and used by disclosure gadget when CPU captures the exception. However, the second question is important regarding the reliability of the methods we use for further analysis. Thus, the purpose of the experiments in this section is not to completely reveal the detailed facts about the zero phenomenon but to understand the true behavior of the instructions issued to ROB. We leverage covert channel and performance counters to study the question.}

\begin{lstlisting}[float=htbp,caption={The effects of P2 on the execution engine.}, label={lst:squash}]
 // %RBX: address of uncached covert channel buffer
 // (%RBX-0x40): address of uncached data
 // *(%RBX-0x40) = %RBX
 // %RAX: address of some other uncached memory
 // %RCX: illegal address whose data is 0x42000
 // ---------------------------------------------
 // Windowing Gadget
     sub %rbx, %rax
     sub %rbx, %rcx
     sub $0x40, %rbx
     movq (%rbx), %rbx
     [movq (%rax, %rbx, 1), %rax] // only for Sec IV.E
 // ---------------------------------------------
 // Speculation Primitive
     movq (%rcx, %rbx, 1), %rcx
 // ---------------------------------------------
 // Disclosure Gadget
     [add $1, %rbx]
     [sub $1, %rbx]
     ...
     movq (%rbx), %rbx
\end{lstlisting}

\bheading{Instruction sequences.}
The instructions of the Disclosure Gadget are independent of the data read by the Speculation Primitive. However, because all instructions in the Speculation Primitive and the Disclosure Gadget are dependent on the data fetched in the Windowing Gadget, the Speculation Primitive and the Disclosure Gadget start at the same time. 

% A sample of the code is shown in \lstref{lst:squash} .The speculation primitive we design is a simple MOV from an illegal address (eg. supervisor-mode address) to a register. Following it is an instruction to touch a covert channel buffer.

% Besides the two instructions, we insert between them a few extra ADD/SUB instructions to change the latency for the covert channel instruction to execute. The inserted instructions  ensure that each of them is dependent on its windowing gadget and the covert channel instruction depends on the last of them. By changing the number of such inserted instructions, we are able to change comparatively how late the covert channel instruction is likely to execute. 
% Notice that the ADD instructions may increase the address too much so that another cacheline is touched. When the number of ADDs is beyond such a limit, we could replace the first ADD with a SUB. For example, a code sequence of "sub \$64, \%rdi" followed by 64 "add \$1, \$rdi" still makes sure \%RDI stores the address to the covert channel buffer.

% To eliminate the interference of other parts of the execution engine such as issuing, a slow data load from memory is put in front of the speculation primitive. Besides, both the speculation primitive and the first ADD instruction is dependent of its data, ensuring that they start execution at the same time when the data becomes available. While they are waiting for the data, the instruction issuing is still going on until the ROB is full. The long latency of memory loading makes sure the execution of following instructions is not delayed to wait for issuing of future instructions.

\bheading{Experiments and expected observations.}
In this test, the framework tunes the number of ADD/SUB instructions inserted in the Disclosure Gadget. If all issued instructions are eventually executed (\ie, not squashed at \phasetwo), we would expect to receive the covert-channel signal regardless of the number of inserted ADD/SUB instructions. Otherwise, the signal should disappear when the number of ADD/SUB instructions increases to a certain threshold.

%, we reload the covert channel buffer and count in 100,000 rounds how many of them show that the buffer is touched, reflecting whether the last MOV instruction is executed. When we delay the covert channel load instruction by inserting a number of ADD/SUB instructions to a certain extent, it will be later than the retirement of the speculation primitive, \ie \phasetwo. Combined with the condition that the issuing of all the instructions in the disclosure gadget is ensured by the windowing gadget, we would like to observe whether the all the instructions could still be executed in this scenario.



\subsection{\phaseone on Execution Engine}
\label{subsec:e1_exec}

\bheading{Test goals.}
In this test, we hope to confirm that \phaseone does not influence other components of the execution engine, \ie, squashing speculative instructions in ROB and/or the altering code fetching in the front end. 

\bheading{Instruction sequences.}
The instruction sequence design is the same as \lstref{lst:squash}. 

\bheading{Experiments and expected observations.}
The overall strategy of the test is to change the latency of \phaseone while fixing the latency of \phasetwo. If the measured speculation window does not change according to \phaseone latency, \phaseone has no effect on the entire execution engine. 

To change the latency of \phaseone, we control the TLB status of the page storing the secret data---by preloading or flushing the TLB entry. In this way, \phaseone of the Speculation Primitive changes accordingly. %With given address translation latency, the data fetching and security check both begin at a certain time. As a result, the latency for the CPU to capture the exception, \ie \phaseone, is also controlled.

To fix \phasetwo latency, one additional memory load instruction is added in the windowing gadget (line 12 of \lstref{lst:squash}), which begins execution at the same time as the Speculation Primitive and the Disclosure Gadget. The goal of this instruction is to delay the retirement of all subsequent instructions, so that the retirement of the Speculation Primitive waits on the retirement of this memory load instruction. In this way, the \phasetwo latency is not determined by the the Speculation Primitive itself, which is changed because the TLB entry of the secret data page is preloaded or flushed, but by the retirement of the memory load instruction. To achieve this goal, the data to be loaded by this instruction is placed in the L2 cache and the TLB of the corresponding page is flushed.  %has a reasonably long retirement latency so that the speculation primitive retires right after it. In the experiments, we leverage a memory load instruction for the purpose and we force its TLB flushed and its data in L2 cache (the illegal data accessed by the speculation primitive has data in L1D). 

%\yz{removing this code is because it is confusing.} One caveat is that this memory load cannot be too slow, because otherwise the speculation window cannot be measured using the Disclosure Gadget once it exceeds the limit of the ROB. To solve this problem, the ADD/SUB instruction in the Disclosure Gadget is replaced with long latency instructions (as long as their latency is constant). \yz{consider illustrating the code}

%we need to replace one or more of the ADD/SUB instructions with instructions demanding more cycles to execute, \eg a memory load with TLB entry present and data in L1. We do not need to know exactly how many cycles it needs since we only need to observe whether the speculation window changes from a differential view.

%Again, the disclosure primitive reloads the covert channel buffer and counts whether the last MOV instruction is executed among 100,000 rounds of tests. 
% With more and more inserted ADD/SUB instructions, the possibility for the last MOV to execute lowers until it is impossible to execute at all. 
%The attack window corresponds to the latency of squashing of ROB, so we observe whether changing the latency of \phaseone by preloading or flushing the TLB entry of the illegal address leads to the change of the attack window.



% Between the speculation primitive and the disclosure gadget, we insert a certain number of extra ADD/SUB instructions to change the latency for the covert channel instruction to execute. The inserted instructions are all dependent on their preceding instruction, including the illegal MOV of speculation primitive. They only begin execution after the illegal data becomes available. The disclosure gadget depends on the last of them. By changing the number of such inserted instructions, we are able to change comparatively how late the covert channel instruction is likely to execute. 





\subsection{Measuring \vulname Exploitability}
\label{subsec:e1_measure}

\bheading{Test goals.} This test aims to determine whether a given variant of \vulname is exploitable, by measuring the relative latency of \phaseone and the fetch of the secret data. If \phaseone comes sooner, the processor is not vulnerable with regard to the underlying Speculation Primitive. 

%Following the study on \phaseone in \secref{subsec:e1_existence} and \secref{subsec:e1_effect}, the most interesting question related to \phaseone is how it determines the exploitability of a potential variant. Thus, a most important test is to find out whether \phaseone could be later than data fetching in the best conditions. Or by other words, whether a potential variant corresponding to a certain cause of exception is exploitable. With the help of \sysname, we try to systematically and comprehensively measure the exploitability of all possible variants as explained in \secref{subsec:instruction_model} and \secref{subsec:exception_plugin}.

\bheading{Instruction sequences.}
As shown in \lstref{lst:exploitability}, the Windowing Gadget is a memory load instruction that retires slowly due to long latency of memory access, but it does not have dependency on the previous instructions, nor does any subsequent instructions depend on it. It is used to ensure that the retirement of the Speculation Primitive (the \phasetwo latency) is sufficiently delayed. %Otherwise, there is a chance for the cases that should capture a correct value (exploitable) or zero value (in-exploitable) to falsely demonstrate no value results (no speculation allowed), although in most cases the disclosure gadget only includes one single instruction to touch the covert channel buffer. The speculation primitive needs to be adapted to the need of the tested variant, \ie the exception cause. In certain cases it may contain two instructions, which is explained in \secref{subsec:instruction_model}. Other parts of the instruction sequence remain the same.

\begin{lstlisting}[float=htbp,caption={Exploitability test with \phaseone measurement.},label={lst:exploitability}]
 // %RBX: address of uncached covert channel buffer
 // (%RBX-0x40): address of uncached data
 // *(%RBX-0x40) = %RBX
 // %RCX: illegal address whose data is 0x42000
 // ---------------------------------------------
 // windowing gadget
     movq %rbx, %rax
     sub $0x40, %rax
     movq (%rax), %rax
 // ---------------------------------------------
 // speculation primitive
     movq (%rcx), %rcx // could be any illegal inst.
 // ---------------------------------------------
 // disclosure gadget
     movq (%rbx, %rcx, 1), %rbx
\end{lstlisting}

\bheading{Experiments and expected observations.}
The same instruction sequence was tested under a variety of conditions, with varying data access latency (cached in L1, L2, or LLC) and address translation latency (whether or not TLB entries are created for the corresponding pages). \sysname is able to enumerate all possible combinations to achieve the optimal condition. In each test, if the Disclosure Primitive receives the correct signal from the covert channel, the vulnerability is exploitable. Otherwise, if a zero signal is received, the vulnerability is not exploitable as the \phaseone latency is shorter than data available latency. However, if no signal can be received, speculation is not allowed. %The test is repeated 100,000 times to improve reliability of the results. 


%The best condition for the tested variant is achieved by making the data fetching latency to be as short as possible compared to \phaseone latency, with the help of \sysname. For example, if the exception is triggered by a memory load, the data is preloaded into L1D. Other conditions like TLB status is set to either accelerate data fetching or to delay exception capturing. When it is not clear how the best condition is achieved, \sysname is able to enumerate all possible settings.

\subsection{Quantitatively Measuring \phaseone Latency}
\label{subsec:e1_change}

\bheading{Test goals.}
This test aims to quantitatively measure the relative latency of \phaseone, compared to data fetching. 

%The overall idea of the measurement of \phaseone latency is that instead of monitoring the architecturally uncatchable event of \phaseone itself, we try to measure the latency for the dummy zero value produced by \phaseone to be provided for following dependent instructions to execute. To measure data fetching latency, we take advantage of the fact that within a given period of time, the total number of instructions that could be executed is constant. Thus, the longer the data fetching latency is, the fewer following dependent instructions could be executed. \yz{not clear}


\begin{lstlisting}[float=htbp,caption={Quantitative measurement of \phaseone latency},captionpos=b,label={lst:framework2}]
 // %RBX: address of uncached covert channel buffer
 // %RCX: illegal address whose data is 0x42000
 // ---------------------------------------------
 // Suppressing Primitive
     [movq (%rax), %rax] // legal access
     [movq (%rax), %rax] // legal access
     ...
     movq (%rax), %rax // suppressing w/ exception
 // ---------------------------------------------
 // Speculation Primitive
     movq (%rcx), %rcx // could be any illegal inst.
 // ---------------------------------------------
 // Disclosure Gadget
     [add $1, %rcx]
     [sub $1, %rcx]
     ...
     movq (%rbx, %rcx, 1), %rcx
\end{lstlisting}

\bheading{Instruction sequences.}
The construction of the instruction sequence is different from other tests as a \textit{Suppressing Primitive} is needed in the test. The Suppressing Primitive precedes all other components in order to conceal the effect of executing the \pluginonename. This is achieved by ensuring that the instructions executed in all other components never retire. In the example of \lstref{lst:framework2}, the Suppressing Primitive is simply an illegal memory load from address 0, but it can also be implemented using conditional branches, indirect jumps, or retpoline. The Suppressing Primitive creates a fixed speculation window for the rest of the instruction sequence to execute. Because it is desired that this speculation window is greater than the one created by the Speculation Primitive, the Suppressing Primitive includes a few memory loads before the faulting instruction and leverages the pointer chasing technique~\cite{pointerchasing} to further enlarge its speculation window. The speculation window cannot be longer than the size of the ROB.

%There could be a chance that one single invalid access does not provide a large enough window for the tested speculation primitive. The solution is to leverage pointer chasing technique to put in the windowing gadget additional dependent legal memory accesses ahead of the invalid access instruction. However, we should not make the window too long either. The reason is that the speculative execution would therefore be limited by the size of ROB instead of the retirement time of the suppressing primitive, making the measurement impossible.

%This is slightly different from traditional concept of exception handling with TSX transaction and signal handler. Typical suppressing methods we leverage include poisoned indirect jump, poisoned conditional branch, Retpoline and another exception. What's more, some side effects of the Suppressing Primitives could be used to perform special tests as explained in \secref{subsec:e1_change}. \yz{hard to understand}

%In addition to its original use of hiding the exeption raised by the speculation primitive, the main purpose of such techniques is to set a time bomb which will terminate the speculative execution after a constant period of time. Thus, the total time for the speculative execution of inner instructions is deterministic and irrelevant to them. The suppressing primitive we pick is an access to an invalid virtual address with no mapping to any physical page. The reason will be explained in \secref{subsec:e1_change_eval}.




A type-II Disclosure Gadget is used; all its instructions depend on the Speculation Primitive. Thus, the Disclosure Gadget only begins execution after the data is returned from the Speculation Primitive, regardless of its correctness. 



% \yx{this paragraph is moved from sec 4 to here, use it as a reference}
% In the code snippet sample in \lstref{lst:framework2} we could see that the tested speculation primitive as well as the covert channel access instruction is wrapped by a certain exception suppressing technique (eg. poisoned indirect jump, poisoned conditional branch, retpoline or another exception). But here the purpose of such techniques is to set a time bomb which will terminate the speculative execution after a constant period of time. Thus, the total time for the speculative execution of inner instructions is deterministic and irrelevant to them. By inserting a certain number of inter-dependent ADD/SUB instruction between the tested speculation primitive and the covert channel access instruction, we delay the beginning of execution of the last instruction due to dependency. And all such ADD/SUB instructions have to wait until the speculation primitive to provide a data, either correct value or zero, to begin execution. We wish to find the maximal number of inserted instructions that still allows the last instruction to execute. And by purposefully forcing a zero is returned by the speculation primitive (eg. by flushing data out of L1 cache when testing the meltdown-US variant), we could thus compute the \phaseone latency as (T(total\_window) - T(add/sub\_latency) * maximal\_inserted\_num). The latency of one add and sub instruction is one cycle. We do not have to calculate the total speculative window to get the \phaseone latency. Instead, we use a differential method to compare it with the latency of a legal data access measured using the same method. Then we could directly know the relative number of cycles between \phaseone and data availability.

% (Preceding: specific purpose due to the method adopted.)
% For the instruction sequences to be used by the second framework, the windowing gadget part should include the instructions specific for the suppressing method chosen. In our implementation we picked wrapping an exception with another exception, whose reason will be explained in later parts. The wrapper instruction we picked is an access to an invalid virtual address with no mapping to any physical page. So the instruction sequence turns into the form of \lstref{lst:framework2}.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{fig/e1_latency.png}
\caption{Illustration of quantitatively measurement of \phaseone latency.}
\label{fig:e1_latency}
\vspace{5pt}
\end{figure}

\bheading{Experiments and expected observations.}
By flushing the secret data to memory, the framework ensures that a zero data is returned by the Speculation Primitive. Let $T_{P1}$ be the number of cycles to retrieve the zero data by the Speculation Primitive, $T_{spec1}$ be the speculation window of the Suppressing Primitive, and $T_{delay}$ be the latency for the Speculation Primitive to begin execution, which are both fixed. The number of inserted instructions in the Disclosure Gadget is tuned to determine $T_{spec2}$, which is the speculation window of the Speculation Primitive. As the Disclosure Gadget starts after the Speculation Primitive has retrieved the data, we have $T_{delay} + T_{P1} + T_{spec2} = T_{spec1}$ (shown in \figref{fig:e1_latency}).

To estimate $T_{P1}$, a control test is run. In the control test, the Speculation Primitive accesses a legal data, which does not trigger exceptions. But still, the execution will be reverted due to the Suppressing Primitive. In this case, the number of cycles to retrieve the legal data is $T_{data}$. With all other conditions unchanged, we have $T_{delay} + T_{data} + T_{spec2'} = T_{spec1}$. Without the need of calculating the exact values of $T_{spec1}$ and $T_{delay}$, the relationship between $T_{data}$ and $T_{P1}$ can be estimated in a differential manner: $T_{data} - T_{P1} = T_{spec2} - T_{spec2'}$.

%We do not have to calculate the total speculative window to get the \phaseone latency. Instead, we use a differential method to compare it with the latency of a legal data fetching, under the same execution conditions (except caching status), measured with the same method. The caching status of the legal data fetching is decided by which level of cache latency is to be measured. The two rounds of tests are identical except whether the condition to trigger an exception is met (\eg whether the US bit in the PTE is set for Meltdown-US test). Then we could know the relative latency in a granularity of cycles between \phaseone and data availability.

% \bheading{Dynamic instruction insertion.}
% A special component in the second framework is that we should be able to dynamically insert ADD/SUB instructions one by one between the tested speculation primitive and the covert channel access instructions until the covert channel is found unable to be touched. In this way, we could find the maximal number of ADD/SUB instructions allowed in the speculative window.

% \bheading{Relative exploitation window measurement.}
% The differential method requires two rounds of test. In the first round, we look for the maximal number of allowed inserted instructions when the covert channel captures only zero value. In the second round, we make the tested instruction legal or be able to return the correct data under the same execution conditions (except caching status) as in the first test. Then by subtracting the two results, we are able to determine the relative latency from \phaseone to the data latency from a certain level of cache.





\subsection{Measure and Change \phasetwo Latency}
\label{subsec:e2_change}

\bheading{Test goals.}
This test aims to determine whether the latency of \phasetwo can be changed, and if so, how. % As \phasetwo happens when the Speculation Primitive retires, the \sysname framework alters the retirement of the Speculation Primitive in a controllable manner, and then observe the changes of the speculation window, which ends when the speculative instructions are squashed.

%Instruction squashing corresponds to the speculation window and \phasetwo corresponds to speculation primitive retirement. Thus, we need to controllably change the latency of speculation primitive retirement while fixing the latency of \phaseone and see how the speculation window changes accordingly.

\begin{lstlisting}[float=htbp,caption={Changing \phasetwo latency.},label={lst:retirement}]
 // %RDI: address of uncached covert channel buffer
 // %RSI: illegal address whose data is 0x42000
 // ---------------------------------------------
 // Windowing Gadget
     movapd \%xmm0, \%xmm1
     addpd \%xmm1, \%xmm0
     [cpuid]
     mulpd \%xmm1, \%xmm0
     ...
     movapd \%xmm0, \%xmm1
     addpd \%xmm1, \%xmm0
     mulpd \%xmm1, \%xmm0
 // ---------------------------------------------
 // Speculation Primitive
     movq (%rsi), %rax
 // ---------------------------------------------
 // Disclosure Gadget
     [add $1, %rax]
     [sub $1, %rax]
     ...
     movq (%rdi, %rax, 1), %rax
\end{lstlisting}

% \ignore{An assumption with the execution model is that when CPU witnesses an exception, it will immediately stop issuing following instructions but begin fetching and issuing exception handler instructions. Thus, we are able to measure the exception capturing latency by monitoring the number of issued micro-ops powered by performance counters. However, as explained above, we can only perform differential analysis. By controlling non-speculative code, the difference in the total number of issued micro-ops is the same as the difference in the number of speculative micro-ops issued.}

\bheading{Instruction sequences.}
%The best way to manipulate the retirement latency is to place in the windowing gadget instructions whose retirement is slow, so that they queue up in ROB. 
As the retirement of the Speculation Primitive only happens after that of the Window Gadget, the strategy is to delay the latter. The Windowing Gadget consists of 25 repeated sequences of three SSE2 instructions: MOVAPD, ADDPD and MULPPD---thus 75 instructions in total. These floating point instructions are slow but can be executed in parallel with the Speculation Primitive and the Disclosure Gadget. Each of these floating point instructions has data dependency on its predecessor. 

To fine tune the retirement of the Speculation Primitive, a CPUID instruction is inserted in the Windowing Gadget. As the CPUID instruction serializes the execution of the instructions before and after it (\ie, no instruction is issued before CPUID retires), only the floating point instructions after CPUID are effective in the Windowing Gadget. Therefore, the retirement of the Speculation Primitive is further delayed if there is CPUID is inserted earlier in the floating point instructions; and vice versa.

%Given the fixed sequence, we control the EFFECTIVE windowing gadget by inserting a CPUID instruction inside the sequence since CPUID serializes execution. For example, if we want no windowing gadget at all with a clean ROB, we insert CPUID at the end of the windowing gadget sequence, right before the speculation primitive. Or if we want a length of 75, we put CPUID at the beginning of the windowing gadget sequence.

The Disclosure Gadget is of type-II. All instructions are dependent on the Speculation Primitive.

%The reason is that we force the TLB availability and cache status to be constant, making the execution time of the speculation primitive to be always the same. We only care about the changing trend of the speculation window but do not need to measure its exact length.

\bheading{Experiments and expected observations.}
For each position in the Windowing Gadget where CPUID is inserted, the framework automatically alter the number of ADD/SUB instructions to identify the speculation window. In this way, the correlation between \phasetwo and the attack window can be observed. It also answers the question whether the attack window can be changed.

%To validate that the Windowing gadget does delay the retirement of Speculation Primitive as expected, Intel Architecture Code Analyzer (IACA) \cite{} was used to perform static analysis on the code sequence. IACA is a tool released by Intel to provide a cycle-accurate estimation of the execution of the instruction sequence on an out-of-order Intel processor, with the knowledge of the internal micro-architecture structures such as execution units and execution ports. 

%It assumes ideal front-end, out-of-order engine and hierarchical memory. Despite reasonable inaccuracy of the estimation, it provides us with a view of the architectural state of instruction execution. 
%A limitation of IACA is that it only considers the back end of a CPU. So the effect of CPUID as a serialization instruction is not rendered correctly. Thus, we need to manually edit the length of windowing gadget instead of relying on CPUID with IACA analysis. 




\subsection{Speculation Primitive as Prefetcher}
\label{subsec:prefetch}
\bheading{Test goals.}
Some Speculation Primitive may only lead to exploitable vulnerability when the data fetching latency is small---data is already cached in the L1 cache. This test aims to determine whether the Speculation Primitive, though failed to extract secret from L2, LLC, or memory, could work as a prefetcher to preload secret data into lower-level caches so as to facilitate future attacks of the same kind.

%By systematic study with experiments, we come to the conclusion that the speculation primitive is able to prefetch data, but such capability is limited by the action of exception handling phase one to stop the execution. \yx{move conclusion to sec 6}

\bheading{Experiments.}
In this test, no Windowing Gadget is needed. The experiment is conducted in three steps: First, the secret data to be accessed by the Speculation Primitive is preloaded (from the shadown virtual address) into LLC or memory. Second, the tested Speculation Primitive and Disclosure Gadget are executed to load the secret data and trigger an exception. Third, the data is reloaded from the shadow address and the latency is measured. 

Two variants of this experiment were tested: (1) The Speculation Primitive is not executed in step 2; (2) The Speculation Primitive is executed 1000 times in step 2.

%In the second step, we try accessing the data with the illegal virtual address and trigger an exception. For each experiment with the data in a certain level of cache or memory, we perform three tests for comparison. The first is not to execute the speculation primitive, as the baseline. The second is to execute the speculation primitive once. The third is to execute the speculation primitive for 1000 times. In the last step, after returning from the exception handler, we do a reload on the data with the legal address and record the reload latency.



